Automating the Removal of Obsolete TODO Comments

TODO comments are very widely used by software developers to describe their pending tasks during software development. However, after performing the task developers sometimes neglect or simply forget to remove the TODO comment, resulting in obsolete TODO comments. These obsolete TODO comments can confuse development teams and may cause the introduction of bugs in the future, decreasing the software's quality and maintainability. In this work, we propose a novel model, named TDCleaner (TODO comment Cleaner), to identify obsolete TODO comments in software projects. TDCleaner can assist developers in just-in-time checking of TODO comments status and avoid leaving obsolete TODO comments. Our approach has two main stages: offline learning and online prediction. During offline learning, we first automatically establish <code_change, todo_comment, commit_msg> training samples and leverage three neural encoders to capture the semantic features of TODO comment, code change and commit message respectively. TDCleaner then automatically learns the correlations and interactions between different encoders to estimate the final status of the TODO comment. For online prediction, we check a TODO comment's status by leveraging the offline trained model to judge the TODO comment's likelihood of being obsolete. We built our dataset by collecting TODO comments from the top-10,000 Python and Java Github repositories and evaluated TDCleaner on them. Extensive experimental results show the promising performance of our model over a set of benchmarks. We also performed an in-the-wild evaluation with real-world software projects, we reported 18 obsolete TODO comments identified by TDCleaner to Github developers and 9 of them have already been confirmed and removed by the developers, demonstrating the practical usage of our approach.

==> fontawesomesymbols-generic.tex <==
\def\faGlass{\faicon{glass}}
\def\faMusic{\faicon{music}}
\def\faSearch{\faicon{search}}
\def\faEnvelopeO{\faicon{envelope-o}}
\def\faHeart{\faicon{heart}}
\def\faStar{\faicon{star}}
\def\faStarO{\faicon{star-o}}
\def\faUser{\faicon{user}}
\def\faFilm{\faicon{film}}
\def\faThLarge{\faicon{th-large}}
\def\faTh{\faicon{th}}
\def\faThList{\faicon{th-list}}
\def\faCheck{\faicon{check}}
\def\faTimes{\faicon{times}}
\def\faSearchPlus{\faicon{search-plus}}
\def\faSearchMinus{\faicon{search-minus}}
\def\faPowerOff{\faicon{power-off}}
\def\faSignal{\faicon{signal}}
\def\faCog{\faicon{cog}}
\def\faTrashO{\faicon{trash-o}}
\def\faHome{\faicon{home}}
\def\faFileO{\faicon{file-o}}
\def\faClockO{\faicon{clock-o}}
\def\faRoad{\faicon{road}}
\def\faDownload{\faicon{download}}
\def\faArrowCircleODown{\faicon{arrow-circle-o-down}}
\def\faArrowCircleOUp{\faicon{arrow-circle-o-up}}
\def\faInbox{\faicon{inbox}}
\def\faPlayCircleO{\faicon{play-circle-o}}
\def\faRepeat{\faicon{repeat}}
\def\faRefresh{\faicon{refresh}}
\def\faListAlt{\faicon{list-alt}}
\def\faLock{\faicon{lock}}
\def\faFlag{\faicon{flag}}
\def\faHeadphones{\faicon{headphones}}
\def\faVolumeOff{\faicon{volume-off}}
\def\faVolumeDown{\faicon{volume-down}}
\def\faVolumeUp{\faicon{volume-up}}
\def\faQrcode{\faicon{qrcode}}
\def\faBarcode{\faicon{barcode}}
\def\faTag{\faicon{tag}}
\def\faTags{\faicon{tags}}
\def\faBook{\faicon{book}}
\def\faBookmark{\faicon{bookmark}}
\def\faPrint{\faicon{print}}
\def\faCamera{\faicon{camera}}
\def\faFont{\faicon{font}}
\def\faBold{\faicon{bold}}
\def\faItalic{\faicon{italic}}
\def\faTextHeight{\faicon{text-height}}
\def\faTextWidth{\faicon{text-width}}
\def\faAlignLeft{\faicon{align-left}}
\def\faAlignCenter{\faicon{align-center}}
\def\faAlignRight{\faicon{align-right}}
\def\faAlignJustify{\faicon{align-justify}}
\def\faList{\faicon{list}}
\def\faOutdent{\faicon{outdent}}
\def\faIndent{\faicon{indent}}
\def\faVideoCamera{\faicon{video-camera}}
\def\faPictureO{\faicon{picture-o}}
\def\faPencil{\faicon{pencil}}
\def\faMapMarker{\faicon{map-marker}}
\def\faAdjust{\faicon{adjust}}
\def\faTint{\faicon{tint}}
\def\faPencilSquareO{\faicon{pencil-square-o}}
\def\faShareSquareO{\faicon{share-square-o}}
\def\faCheckSquareO{\faicon{check-square-o}}
\def\faArrows{\faicon{arrows}}
\def\faStepBackward{\faicon{step-backward}}
\def\faFastBackward{\faicon{fast-backward}}
\def\faBackward{\faicon{backward}}
\def\faPlay{\faicon{play}}
\def\faPause{\faicon{pause}}
\def\faStop{\faicon{stop}}
\def\faForward{\faicon{forward}}
\def\faFastForward{\faicon{fast-forward}}
\def\faStepForward{\faicon{step-forward}}
\def\faEject{\faicon{eject}}
\def\faChevronLeft{\faicon{chevron-left}}
\def\faChevronRight{\faicon{chevron-right}}
\def\faPlusCircle{\faicon{plus-circle}}
\def\faMinusCircle{\faicon{minus-circle}}
\def\faTimesCircle{\faicon{times-circle}}
\def\faCheckCircle{\faicon{check-circle}}
\def\faQuestionCircle{\faicon{question-circle}}
\def\faInfoCircle{\faicon{info-circle}}
\def\faCrosshairs{\faicon{crosshairs}}
\def\faTimesCircleO{\faicon{times-circle-o}}
\def\faCheckCircleO{\faicon{check-circle-o}}
\def\faBan{\faicon{ban}}
\def\faArrowLeft{\faicon{arrow-left}}
\def\faArrowRight{\faicon{arrow-right}}
\def\faArrowUp{\faicon{arrow-up}}
\def\faArrowDown{\faicon{arrow-down}}
\def\faShare{\faicon{share}}
\def\faExpand{\faicon{expand}}
\def\faCompress{\faicon{compress}}
\def\faPlus{\faicon{plus}}
\def\faMinus{\faicon{minus}}
\def\faAsterisk{\faicon{asterisk}}
\def\faExclamationCircle{\faicon{exclamation-circle}}
\def\faGift{\faicon{gift}}
\def\faLeaf{\faicon{leaf}}
\def\faFire{\faicon{fire}}
\def\faEye{\faicon{eye}}
\def\faEyeSlash{\faicon{eye-slash}}
\def\faExclamationTriangle{\faicon{exclamation-triangle}}
\def\faPlane{\faicon{plane}}
\def\faCalendar{\faicon{calendar}}
\def\faRandom{\faicon{random}}
\def\faComment{\faicon{comment}}
\def\faMagnet{\faicon{magnet}}
\def\faChevronUp{\faicon{chevron-up}}
\def\faChevronDown{\faicon{chevron-down}}
\def\faRetweet{\faicon{retweet}}
\def\faShoppingCart{\faicon{shopping-cart}}
\def\faFolder{\faicon{folder}}
\def\faFolderOpen{\faicon{folder-open}}
\def\faArrowsV{\faicon{arrows-v}}
\def\faArrowsH{\faicon{arrows-h}}
\def\faBarChart{\faicon{bar-chart}}
\def\faTwitterSquare{\faicon{twitter-square}}
\def\faFacebookSquare{\faicon{facebook-square}}
\def\faCameraRetro{\faicon{camera-retro}}
\def\faKey{\faicon{key}}
\def\faCogs{\faicon{cogs}}
\def\faComments{\faicon{comments}}
\def\faThumbsOUp{\faicon{thumbs-o-up}}
\def\faThumbsODown{\faicon{thumbs-o-down}}
\def\faStarHalf{\faicon{star-half}}
\def\faHeartO{\faicon{heart-o}}
\def\faSignOut{\faicon{sign-out}}
\def\faLinkedinSquare{\faicon{linkedin-square}}
\def\faThumbTack{\faicon{thumb-tack}}
\def\faExternalLink{\faicon{external-link}}
\def\faSignIn{\faicon{sign-in}}
\def\faTrophy{\faicon{trophy}}
\def\faGithubSquare{\faicon{github-square}}
\def\faUpload{\faicon{upload}}
\def\faLemonO{\faicon{lemon-o}}
\def\faPhone{\faicon{phone}}
\def\faSquareO{\faicon{square-o}}
\def\faBookmarkO{\faicon{bookmark-o}}
\def\faPhoneSquare{\faicon{phone-square}}
\def\faTwitter{\faicon{twitter}}
\def\faFacebook{\faicon{facebook}}
\def\faGithub{\faicon{github}}
\def\faUnlock{\faicon{unlock}}
\def\faCreditCard{\faicon{credit-card}}
\def\faRss{\faicon{rss}}
\def\faHddO{\faicon{hdd-o}}
\def\faBullhorn{\faicon{bullhorn}}
\def\faBell{\faicon{bell}}
\def\faCertificate{\faicon{certificate}}
\def\faHandORight{\faicon{hand-o-right}}
\def\faHandOLeft{\faicon{hand-o-left}}
\def\faHandOUp{\faicon{hand-o-up}}
\def\faHandODown{\faicon{hand-o-down}}
\def\faArrowCircleLeft{\faicon{arrow-circle-left}}
\def\faArrowCircleRight{\faicon{arrow-circle-right}}
\def\faArrowCircleUp{\faicon{arrow-circle-up}}
\def\faArrowCircleDown{\faicon{arrow-circle-down}}
\def\faGlobe{\faicon{globe}}
\def\faWrench{\faicon{wrench}}
\def\faTasks{\faicon{tasks}}
\def\faFilter{\faicon{filter}}
\def\faBriefcase{\faicon{briefcase}}
\def\faArrowsAlt{\faicon{arrows-alt}}
\def\faUsers{\faicon{users}}
\def\faLink{\faicon{link}}
\def\faCloud{\faicon{cloud}}
\def\faFlask{\faicon{flask}}
\def\faScissors{\faicon{scissors}}
\def\faFilesO{\faicon{files-o}}
\def\faPaperclip{\faicon{paperclip}}
\def\faFloppyO{\faicon{floppy-o}}
\def\faSquare{\faicon{square}}
\def\faBars{\faicon{bars}}
\def\faListUl{\faicon{list-ul}}
\def\faListOl{\faicon{list-ol}}
\def\faStrikethrough{\faicon{strikethrough}}
\def\faUnderline{\faicon{underline}}
\def\faTable{\faicon{table}}
\def\faMagic{\faicon{magic}}
\def\faTruck{\faicon{truck}}
\def\faPinterest{\faicon{pinterest}}
\def\faPinterestSquare{\faicon{pinterest-square}}
\def\faGooglePlusSquare{\faicon{google-plus-square}}
\def\faGooglePlus{\faicon{google-plus}}
\def\faMoney{\faicon{money}}
\def\faCaretDown{\faicon{caret-down}}
\def\faCaretUp{\faicon{caret-up}}
\def\faCaretLeft{\faicon{caret-left}}
\def\faCaretRight{\faicon{caret-right}}
\def\faColumns{\faicon{columns}}
\def\faSort{\faicon{sort}}
\def\faSortDesc{\faicon{sort-desc}}
\def\faSortAsc{\faicon{sort-asc}}
\def\faEnvelope{\faicon{envelope}}
\def\faLinkedin{\faicon{linkedin}}
\def\faUndo{\faicon{undo}}
\def\faGavel{\faicon{gavel}}
\def\faTachometer{\faicon{tachometer}}
\def\faCommentO{\faicon{comment-o}}
\def\faCommentsO{\faicon{comments-o}}
\def\faBolt{\faicon{bolt}}
\def\faSitemap{\faicon{sitemap}}
\def\faUmbrella{\faicon{umbrella}}
\def\faClipboard{\faicon{clipboard}}
\def\faLightbulbO{\faicon{lightbulb-o}}
\def\faExchange{\faicon{exchange}}
\def\faCloudDownload{\faicon{cloud-download}}
\def\faCloudUpload{\faicon{cloud-upload}}
\def\faUserMd{\faicon{user-md}}
\def\faStethoscope{\faicon{stethoscope}}
\def\faSuitcase{\faicon{suitcase}}
\def\faBellO{\faicon{bell-o}}
\def\faCoffee{\faicon{coffee}}
\def\faCutlery{\faicon{cutlery}}
\def\faFileTextO{\faicon{file-text-o}}
\def\faBuildingO{\faicon{building-o}}
\def\faHospitalO{\faicon{hospital-o}}
\def\faAmbulance{\faicon{ambulance}}
\def\faMedkit{\faicon{medkit}}
\def\faFighterJet{\faicon{fighter-jet}}
\def\faBeer{\faicon{beer}}
\def\faHSquare{\faicon{h-square}}
\def\faPlusSquare{\faicon{plus-square}}
\def\faAngleDoubleLeft{\faicon{angle-double-left}}
\def\faAngleDoubleRight{\faicon{angle-double-right}}
\def\faAngleDoubleUp{\faicon{angle-double-up}}
\def\faAngleDoubleDown{\faicon{angle-double-down}}
\def\faAngleLeft{\faicon{angle-left}}
\def\faAngleRight{\faicon{angle-right}}
\def\faAngleUp{\faicon{angle-up}}
\def\faAngleDown{\faicon{angle-down}}
\def\faDesktop{\faicon{desktop}}
\def\faLaptop{\faicon{laptop}}
\def\faTablet{\faicon{tablet}}
\def\faMobile{\faicon{mobile}}
\def\faCircleO{\faicon{circle-o}}
\def\faQuoteLeft{\faicon{quote-left}}
\def\faQuoteRight{\faicon{quote-right}}
\def\faSpinner{\faicon{spinner}}
\def\faCircle{\faicon{circle}}
\def\faReply{\faicon{reply}}
\def\faGithubAlt{\faicon{github-alt}}
\def\faFolderO{\faicon{folder-o}}
\def\faFolderOpenO{\faicon{folder-open-o}}
\def\faSmileO{\faicon{smile-o}}
\def\faFrownO{\faicon{frown-o}}
\def\faMehO{\faicon{meh-o}}
\def\faGamepad{\faicon{gamepad}}
\def\faKeyboardO{\faicon{keyboard-o}}
\def\faFlagO{\faicon{flag-o}}
\def\faFlagCheckered{\faicon{flag-checkered}}
\def\faTerminal{\faicon{terminal}}
\def\faCode{\faicon{code}}
\def\faReplyAll{\faicon{reply-all}}
\def\faStarHalfO{\faicon{star-half-o}}
\def\faLocationArrow{\faicon{location-arrow}}
\def\faCrop{\faicon{crop}}
\def\faCodeFork{\faicon{code-fork}}
\def\faChainBroken{\faicon{chain-broken}}
\def\faQuestion{\faicon{question}}
\def\faInfo{\faicon{info}}
\def\faExclamation{\faicon{exclamation}}
\def\faSuperscript{\faicon{superscript}}
\def\faSubscript{\faicon{subscript}}
\def\faEraser{\faicon{eraser}}
\def\faPuzzlePiece{\faicon{puzzle-piece}}
\def\faMicrophone{\faicon{microphone}}
\def\faMicrophoneSlash{\faicon{microphone-slash}}
\def\faShield{\faicon{shield}}
\def\faCalendarO{\faicon{calendar-o}}
\def\faFireExtinguisher{\faicon{fire-extinguisher}}
\def\faRocket{\faicon{rocket}}
\def\faMaxcdn{\faicon{maxcdn}}
\def\faChevronCircleLeft{\faicon{chevron-circle-left}}
\def\faChevronCircleRight{\faicon{chevron-circle-right}}
\def\faChevronCircleUp{\faicon{chevron-circle-up}}
\def\faChevronCircleDown{\faicon{chevron-circle-down}}
\def\faHtml5{\faicon{html5}}
\def\faCss3{\faicon{css3}}
\def\faAnchor{\faicon{anchor}}
\def\faUnlockAlt{\faicon{unlock-alt}}
\def\faBullseye{\faicon{bullseye}}
\def\faEllipsisH{\faicon{ellipsis-h}}
\def\faEllipsisV{\faicon{ellipsis-v}}
\def\faRssSquare{\faicon{rss-square}}
\def\faPlayCircle{\faicon{play-circle}}
\def\faTicket{\faicon{ticket}}
\def\faMinusSquare{\faicon{minus-square}}
\def\faMinusSquareO{\faicon{minus-square-o}}
\def\faLevelUp{\faicon{level-up}}
\def\faLevelDown{\faicon{level-down}}
\def\faCheckSquare{\faicon{check-square}}
\def\faPencilSquare{\faicon{pencil-square}}
\def\faExternalLinkSquare{\faicon{external-link-square}}
\def\faShareSquare{\faicon{share-square}}
\def\faCompass{\faicon{compass}}
\def\faCaretSquareODown{\faicon{caret-square-o-down}}
\def\faCaretSquareOUp{\faicon{caret-square-o-up}}
\def\faCaretSquareORight{\faicon{caret-square-o-right}}
\def\faEur{\faicon{eur}}
\def\faGbp{\faicon{gbp}}
\def\faUsd{\faicon{usd}}
\def\faInr{\faicon{inr}}
\def\faJpy{\faicon{jpy}}
\def\faRub{\faicon{rub}}
\def\faKrw{\faicon{krw}}
\def\faBtc{\faicon{btc}}
\def\faFile{\faicon{file}}
\def\faFileText{\faicon{file-text}}
\def\faSortAlphaAsc{\faicon{sort-alpha-asc}}
\def\faSortAlphaDesc{\faicon{sort-alpha-desc}}
\def\faSortAmountAsc{\faicon{sort-amount-asc}}
\def\faSortAmountDesc{\faicon{sort-amount-desc}}
\def\faSortNumericAsc{\faicon{sort-numeric-asc}}
\def\faSortNumericDesc{\faicon{sort-numeric-desc}}
\def\faThumbsUp{\faicon{thumbs-up}}
\def\faThumbsDown{\faicon{thumbs-down}}
\def\faYoutubeSquare{\faicon{youtube-square}}
\def\faYoutube{\faicon{youtube}}
\def\faXing{\faicon{xing}}
\def\faXingSquare{\faicon{xing-square}}
\def\faYoutubePlay{\faicon{youtube-play}}
\def\faDropbox{\faicon{dropbox}}
\def\faStackOverflow{\faicon{stack-overflow}}
\def\faInstagram{\faicon{instagram}}
\def\faFlickr{\faicon{flickr}}
\def\faAdn{\faicon{adn}}
\def\faBitbucket{\faicon{bitbucket}}
\def\faBitbucketSquare{\faicon{bitbucket-square}}
\def\faTumblr{\faicon{tumblr}}
\def\faTumblrSquare{\faicon{tumblr-square}}
\def\faLongArrowDown{\faicon{long-arrow-down}}
\def\faLongArrowUp{\faicon{long-arrow-up}}
\def\faLongArrowLeft{\faicon{long-arrow-left}}
\def\faLongArrowRight{\faicon{long-arrow-right}}
\def\faApple{\faicon{apple}}
\def\faWindows{\faicon{windows}}
\def\faAndroid{\faicon{android}}
\def\faLinux{\faicon{linux}}
\def\faDribbble{\faicon{dribbble}}
\def\faSkype{\faicon{skype}}
\def\faFoursquare{\faicon{foursquare}}
\def\faTrello{\faicon{trello}}
\def\faFemale{\faicon{female}}
\def\faMale{\faicon{male}}
\def\faGratipay{\faicon{gratipay}}
\def\faSunO{\faicon{sun-o}}
\def\faMoonO{\faicon{moon-o}}
\def\faArchive{\faicon{archive}}
\def\faBug{\faicon{bug}}
\def\faVk{\faicon{vk}}
\def\faWeibo{\faicon{weibo}}
\def\faRenren{\faicon{renren}}
\def\faPagelines{\faicon{pagelines}}
\def\faStackExchange{\faicon{stack-exchange}}
\def\faArrowCircleORight{\faicon{arrow-circle-o-right}}
\def\faArrowCircleOLeft{\faicon{arrow-circle-o-left}}
\def\faCaretSquareOLeft{\faicon{caret-square-o-left}}
\def\faDotCircleO{\faicon{dot-circle-o}}
\def\faWheelchair{\faicon{wheelchair}}
\def\faVimeoSquare{\faicon{vimeo-square}}
\def\faTry{\faicon{try}}
\def\faPlusSquareO{\faicon{plus-square-o}}
\def\faSpaceShuttle{\faicon{space-shuttle}}
\def\faSlack{\faicon{slack}}
\def\faEnvelopeSquare{\faicon{envelope-square}}
\def\faWordpress{\faicon{wordpress}}
\def\faOpenid{\faicon{openid}}
\def\faUniversity{\faicon{university}}
\def\faGraduationCap{\faicon{graduation-cap}}
\def\faYahoo{\faicon{yahoo}}
\def\faGoogle{\faicon{google}}
\def\faReddit{\faicon{reddit}}
\def\faRedditSquare{\faicon{reddit-square}}
\def\faStumbleuponCircle{\faicon{stumbleupon-circle}}
\def\faStumbleupon{\faicon{stumbleupon}}
\def\faDelicious{\faicon{delicious}}
\def\faDigg{\faicon{digg}}
\def\faPiedPiperPp{\faicon{pied-piper-pp}}
\def\faPiedPiperAlt{\faicon{pied-piper-alt}}
\def\faDrupal{\faicon{drupal}}
\def\faJoomla{\faicon{joomla}}
\def\faLanguage{\faicon{language}}
\def\faFax{\faicon{fax}}
\def\faBuilding{\faicon{building}}
\def\faChild{\faicon{child}}
\def\faPaw{\faicon{paw}}
\def\faSpoon{\faicon{spoon}}
\def\faCube{\faicon{cube}}
\def\faCubes{\faicon{cubes}}
\def\faBehance{\faicon{behance}}
\def\faBehanceSquare{\faicon{behance-square}}
\def\faSteam{\faicon{steam}}
\def\faSteamSquare{\faicon{steam-square}}
\def\faRecycle{\faicon{recycle}}
\def\faCar{\faicon{car}}
\def\faTaxi{\faicon{taxi}}
\def\faTree{\faicon{tree}}
\def\faSpotify{\faicon{spotify}}
\def\faDeviantart{\faicon{deviantart}}
\def\faSoundcloud{\faicon{soundcloud}}
\def\faDatabase{\faicon{database}}
\def\faFilePdfO{\faicon{file-pdf-o}}
\def\faFileWordO{\faicon{file-word-o}}
\def\faFileExcelO{\faicon{file-excel-o}}
\def\faFilePowerpointO{\faicon{file-powerpoint-o}}
\def\faFileImageO{\faicon{file-image-o}}
\def\faFileArchiveO{\faicon{file-archive-o}}
\def\faFileAudioO{\faicon{file-audio-o}}
\def\faFileVideoO{\faicon{file-video-o}}
\def\faFileCodeO{\faicon{file-code-o}}
\def\faVine{\faicon{vine}}
\def\faCodepen{\faicon{codepen}}
\def\faJsfiddle{\faicon{jsfiddle}}
\def\faLifeRing{\faicon{life-ring}}
\def\faCircleONotch{\faicon{circle-o-notch}}
\def\faRebel{\faicon{rebel}}
\def\faEmpire{\faicon{empire}}
\def\faGitSquare{\faicon{git-square}}
\def\faGit{\faicon{git}}
\def\faHackerNews{\faicon{hacker-news}}
\def\faTencentWeibo{\faicon{tencent-weibo}}
\def\faQq{\faicon{qq}}
\def\faWeixin{\faicon{weixin}}
\def\faPaperPlane{\faicon{paper-plane}}
\def\faPaperPlaneO{\faicon{paper-plane-o}}
\def\faHistory{\faicon{history}}
\def\faCircleThin{\faicon{circle-thin}}
\def\faHeader{\faicon{header}}
\def\faParagraph{\faicon{paragraph}}
\def\faSliders{\faicon{sliders}}
\def\faShareAlt{\faicon{share-alt}}
\def\faShareAltSquare{\faicon{share-alt-square}}
\def\faBomb{\faicon{bomb}}
\def\faFutbolO{\faicon{futbol-o}}
\def\faTty{\faicon{tty}}
\def\faBinoculars{\faicon{binoculars}}
\def\faPlug{\faicon{plug}}
\def\faSlideshare{\faicon{slideshare}}
\def\faTwitch{\faicon{twitch}}
\def\faYelp{\faicon{yelp}}
\def\faNewspaperO{\faicon{newspaper-o}}
\def\faWifi{\faicon{wifi}}
\def\faCalculator{\faicon{calculator}}
\def\faPaypal{\faicon{paypal}}
\def\faGoogleWallet{\faicon{google-wallet}}
\def\faCcVisa{\faicon{cc-visa}}
\def\faCcMastercard{\faicon{cc-mastercard}}
\def\faCcDiscover{\faicon{cc-discover}}
\def\faCcAmex{\faicon{cc-amex}}
\def\faCcPaypal{\faicon{cc-paypal}}
\def\faCcStripe{\faicon{cc-stripe}}
\def\faBellSlash{\faicon{bell-slash}}
\def\faBellSlashO{\faicon{bell-slash-o}}
\def\faTrash{\faicon{trash}}
\def\faCopyright{\faicon{copyright}}
\def\faAt{\faicon{at}}
\def\faEyedropper{\faicon{eyedropper}}
\def\faPaintBrush{\faicon{paint-brush}}
\def\faBirthdayCake{\faicon{birthday-cake}}
\def\faAreaChart{\faicon{area-chart}}
\def\faPieChart{\faicon{pie-chart}}
\def\faLineChart{\faicon{line-chart}}
\def\faLastfm{\faicon{lastfm}}
\def\faLastfmSquare{\faicon{lastfm-square}}
\def\faToggleOff{\faicon{toggle-off}}
\def\faToggleOn{\faicon{toggle-on}}
\def\faBicycle{\faicon{bicycle}}
\def\faBus{\faicon{bus}}
\def\faIoxhost{\faicon{ioxhost}}
\def\faAngellist{\faicon{angellist}}
\def\faCc{\faicon{cc}}
\def\faIls{\faicon{ils}}
\def\faMeanpath{\faicon{meanpath}}
\def\faBuysellads{\faicon{buysellads}}
\def\faConnectdevelop{\faicon{connectdevelop}}
\def\faDashcube{\faicon{dashcube}}
\def\faForumbee{\faicon{forumbee}}
\def\faLeanpub{\faicon{leanpub}}
\def\faSellsy{\faicon{sellsy}}
\def\faShirtsinbulk{\faicon{shirtsinbulk}}
\def\faSimplybuilt{\faicon{simplybuilt}}
\def\faSkyatlas{\faicon{skyatlas}}
\def\faCartPlus{\faicon{cart-plus}}
\def\faCartArrowDown{\faicon{cart-arrow-down}}
\def\faDiamond{\faicon{diamond}}
\def\faShip{\faicon{ship}}
\def\faUserSecret{\faicon{user-secret}}
\def\faMotorcycle{\faicon{motorcycle}}
\def\faStreetView{\faicon{street-view}}
\def\faHeartbeat{\faicon{heartbeat}}
\def\faVenus{\faicon{venus}}
\def\faMars{\faicon{mars}}
\def\faMercury{\faicon{mercury}}
\def\faTransgender{\faicon{transgender}}
\def\faTransgenderAlt{\faicon{transgender-alt}}
\def\faVenusDouble{\faicon{venus-double}}
\def\faMarsDouble{\faicon{mars-double}}
\def\faVenusMars{\faicon{venus-mars}}
\def\faMarsStroke{\faicon{mars-stroke}}
\def\faMarsStrokeV{\faicon{mars-stroke-v}}
\def\faMarsStrokeH{\faicon{mars-stroke-h}}
\def\faNeuter{\faicon{neuter}}
\def\faGenderless{\faicon{genderless}}
\def\faFacebookOfficial{\faicon{facebook-official}}
\def\faPinterestP{\faicon{pinterest-p}}
\def\faWhatsapp{\faicon{whatsapp}}
\def\faServer{\faicon{server}}
\def\faUserPlus{\faicon{user-plus}}
\def\faUserTimes{\faicon{user-times}}
\def\faBed{\faicon{bed}}
\def\faViacoin{\faicon{viacoin}}
\def\faTrain{\faicon{train}}
\def\faSubway{\faicon{subway}}
\def\faMedium{\faicon{medium}}
\def\faYCombinator{\faicon{y-combinator}}
\def\faOptinMonster{\faicon{optin-monster}}
\def\faOpencart{\faicon{opencart}}
\def\faExpeditedssl{\faicon{expeditedssl}}
\def\faBatteryFull{\faicon{battery-full}}
\def\faBatteryThreeQuarters{\faicon{battery-three-quarters}}
\def\faBatteryHalf{\faicon{battery-half}}
\def\faBatteryQuarter{\faicon{battery-quarter}}
\def\faBatteryEmpty{\faicon{battery-empty}}
\def\faMousePointer{\faicon{mouse-pointer}}
\def\faICursor{\faicon{i-cursor}}
\def\faObjectGroup{\faicon{object-group}}
\def\faObjectUngroup{\faicon{object-ungroup}}
\def\faStickyNote{\faicon{sticky-note}}
\def\faStickyNoteO{\faicon{sticky-note-o}}
\def\faCcJcb{\faicon{cc-jcb}}
\def\faCcDinersClub{\faicon{cc-diners-club}}
\def\faClone{\faicon{clone}}
\def\faBalanceScale{\faicon{balance-scale}}
\def\faHourglassO{\faicon{hourglass-o}}
\def\faHourglassStart{\faicon{hourglass-start}}
\def\faHourglassHalf{\faicon{hourglass-half}}
\def\faHourglassEnd{\faicon{hourglass-end}}
\def\faHourglass{\faicon{hourglass}}
\def\faHandRockO{\faicon{hand-rock-o}}
\def\faHandPaperO{\faicon{hand-paper-o}}
\def\faHandScissorsO{\faicon{hand-scissors-o}}
\def\faHandLizardO{\faicon{hand-lizard-o}}
\def\faHandSpockO{\faicon{hand-spock-o}}
\def\faHandPointerO{\faicon{hand-pointer-o}}
\def\faHandPeaceO{\faicon{hand-peace-o}}
\def\faTrademark{\faicon{trademark}}
\def\faRegistered{\faicon{registered}}
\def\faCreativeCommons{\faicon{creative-commons}}
\def\faGg{\faicon{gg}}
\def\faGgCircle{\faicon{gg-circle}}
\def\faTripadvisor{\faicon{tripadvisor}}
\def\faOdnoklassniki{\faicon{odnoklassniki}}
\def\faOdnoklassnikiSquare{\faicon{odnoklassniki-square}}
\def\faGetPocket{\faicon{get-pocket}}
\def\faWikipediaW{\faicon{wikipedia-w}}
\def\faSafari{\faicon{safari}}
\def\faChrome{\faicon{chrome}}
\def\faFirefox{\faicon{firefox}}
\def\faOpera{\faicon{opera}}
\def\faInternetExplorer{\faicon{internet-explorer}}
\def\faTelevision{\faicon{television}}
\def\faContao{\faicon{contao}}
\def\fa500Px{\faicon{500px}}
\def\faAmazon{\faicon{amazon}}
\def\faCalendarPlusO{\faicon{calendar-plus-o}}
\def\faCalendarMinusO{\faicon{calendar-minus-o}}
\def\faCalendarTimesO{\faicon{calendar-times-o}}
\def\faCalendarCheckO{\faicon{calendar-check-o}}
\def\faIndustry{\faicon{industry}}
\def\faMapPin{\faicon{map-pin}}
\def\faMapSigns{\faicon{map-signs}}
\def\faMapO{\faicon{map-o}}
\def\faMap{\faicon{map}}
\def\faCommenting{\faicon{commenting}}
\def\faCommentingO{\faicon{commenting-o}}
\def\faHouzz{\faicon{houzz}}
\def\faVimeo{\faicon{vimeo}}
\def\faBlackTie{\faicon{black-tie}}
\def\faFonticons{\faicon{fonticons}}
\def\faRedditAlien{\faicon{reddit-alien}}
\def\faEdge{\faicon{edge}}
\def\faCreditCardAlt{\faicon{credit-card-alt}}
\def\faCodiepie{\faicon{codiepie}}
\def\faModx{\faicon{modx}}
\def\faFortAwesome{\faicon{fort-awesome}}
\def\faUsb{\faicon{usb}}
\def\faProductHunt{\faicon{product-hunt}}
\def\faMixcloud{\faicon{mixcloud}}
\def\faScribd{\faicon{scribd}}
\def\faPauseCircle{\faicon{pause-circle}}
\def\faPauseCircleO{\faicon{pause-circle-o}}
\def\faStopCircle{\faicon{stop-circle}}
\def\faStopCircleO{\faicon{stop-circle-o}}
\def\faShoppingBag{\faicon{shopping-bag}}
\def\faShoppingBasket{\faicon{shopping-basket}}
\def\faHashtag{\faicon{hashtag}}
\def\faBluetooth{\faicon{bluetooth}}
\def\faBluetoothB{\faicon{bluetooth-b}}
\def\faPercent{\faicon{percent}}
\def\faGitlab{\faicon{gitlab}}
\def\faWpbeginner{\faicon{wpbeginner}}
\def\faWpforms{\faicon{wpforms}}
\def\faEnvira{\faicon{envira}}
\def\faUniversalAccess{\faicon{universal-access}}
\def\faWheelchairAlt{\faicon{wheelchair-alt}}
\def\faQuestionCircleO{\faicon{question-circle-o}}
\def\faBlind{\faicon{blind}}
\def\faAudioDescription{\faicon{audio-description}}
\def\faVolumeControlPhone{\faicon{volume-control-phone}}
\def\faBraille{\faicon{braille}}
\def\faAssistiveListeningSystems{\faicon{assistive-listening-systems}}
\def\faAmericanSignLanguageInterpreting{\faicon{american-sign-language-interpreting}}
\def\faDeaf{\faicon{deaf}}
\def\faGlide{\faicon{glide}}
\def\faGlideG{\faicon{glide-g}}
\def\faSignLanguage{\faicon{sign-language}}
\def\faLowVision{\faicon{low-vision}}
\def\faViadeo{\faicon{viadeo}}
\def\faViadeoSquare{\faicon{viadeo-square}}
\def\faSnapchat{\faicon{snapchat}}
\def\faSnapchatGhost{\faicon{snapchat-ghost}}
\def\faSnapchatSquare{\faicon{snapchat-square}}
\def\faPiedPiper{\faicon{pied-piper}}
\def\faFirstOrder{\faicon{first-order}}
\def\faYoast{\faicon{yoast}}
\def\faThemeisle{\faicon{themeisle}}
\def\faGooglePlusOfficial{\faicon{google-plus-official}}
\def\faFontAwesome{\faicon{font-awesome}}
% aliases
\def\faCny{\faicon{cny}}\expandafter\def\csname faicon@cny\endcsname{\faicon{jpy}}
\def\faYCombinatorSquare{\faicon{y-combinator-square}}\expandafter\def\csname faicon@y-combinator-square\endcsname{\faicon{hacker-news}}
\def\faCab{\faicon{cab}}\expandafter\def\csname faicon@cab\endcsname{\faicon{taxi}}
\def\faToggleUp{\faicon{toggle-up}}\expandafter\def\csname faicon@toggle-up\endcsname{\faicon{caret-square-o-up}}
\def\faLifeBuoy{\faicon{life-buoy}}\expandafter\def\csname faicon@life-buoy\endcsname{\faicon{life-ring}}
\def\faFileZipO{\faicon{file-zip-o}}\expandafter\def\csname faicon@file-zip-o\endcsname{\faicon{file-archive-o}}
\def\faBitcoin{\faicon{bitcoin}}\expandafter\def\csname faicon@bitcoin\endcsname{\faicon{btc}}
\def\faAutomobile{\faicon{automobile}}\expandafter\def\csname faicon@automobile\endcsname{\faicon{car}}
\def\faPaste{\faicon{paste}}\expandafter\def\csname faicon@paste\endcsname{\faicon{clipboard}}
\def\faResistance{\faicon{resistance}}\expandafter\def\csname faicon@resistance\endcsname{\faicon{rebel}}
\def\faCopy{\faicon{copy}}\expandafter\def\csname faicon@copy\endcsname{\faicon{files-o}}
\def\faIntersex{\faicon{intersex}}\expandafter\def\csname faicon@intersex\endcsname{\faicon{transgender}}
\def\faHardOfHearing{\faicon{hard-of-hearing}}\expandafter\def\csname faicon@hard-of-hearing\endcsname{\faicon{deaf}}
\def\faMailReply{\faicon{mail-reply}}\expandafter\def\csname faicon@mail-reply\endcsname{\faicon{reply}}
\def\faSortDown{\faicon{sort-down}}\expandafter\def\csname faicon@sort-down\endcsname{\faicon{sort-desc}}
\def\faGe{\faicon{ge}}\expandafter\def\csname faicon@ge\endcsname{\faicon{empire}}
\def\faBattery2{\faicon{battery-2}}\expandafter\def\csname faicon@battery-2\endcsname{\faicon{battery-half}}
\def\faHandStopO{\faicon{hand-stop-o}}\expandafter\def\csname faicon@hand-stop-o\endcsname{\faicon{hand-paper-o}}
\def\faGroup{\faicon{group}}\expandafter\def\csname faicon@group\endcsname{\faicon{users}}
\def\faRotateRight{\faicon{rotate-right}}\expandafter\def\csname faicon@rotate-right\endcsname{\faicon{repeat}}
\def\faWon{\faicon{won}}\expandafter\def\csname faicon@won\endcsname{\faicon{krw}}
\def\faFa{\faicon{fa}}\expandafter\def\csname faicon@fa\endcsname{\faicon{font-awesome}}
\def\faHourglass3{\faicon{hourglass-3}}\expandafter\def\csname faicon@hourglass-3\endcsname{\faicon{hourglass-end}}
\def\faStarHalfEmpty{\faicon{star-half-empty}}\expandafter\def\csname faicon@star-half-empty\endcsname{\faicon{star-half-o}}
\def\faCut{\faicon{cut}}\expandafter\def\csname faicon@cut\endcsname{\faicon{scissors}}
\def\faToggleDown{\faicon{toggle-down}}\expandafter\def\csname faicon@toggle-down\endcsname{\faicon{caret-square-o-down}}
\def\faGooglePlusCircle{\faicon{google-plus-circle}}\expandafter\def\csname faicon@google-plus-circle\endcsname{\faicon{google-plus-official}}
\def\faSheqel{\faicon{sheqel}}\expandafter\def\csname faicon@sheqel\endcsname{\faicon{ils}}
\def\faDashboard{\faicon{dashboard}}\expandafter\def\csname faicon@dashboard\endcsname{\faicon{tachometer}}
\def\faSend{\faicon{send}}\expandafter\def\csname faicon@send\endcsname{\faicon{paper-plane}}
\def\faYc{\faicon{yc}}\expandafter\def\csname faicon@yc\endcsname{\faicon{y-combinator}}
\def\faToggleLeft{\faicon{toggle-left}}\expandafter\def\csname faicon@toggle-left\endcsname{\faicon{caret-square-o-left}}
\def\faWarning{\faicon{warning}}\expandafter\def\csname faicon@warning\endcsname{\faicon{exclamation-triangle}}
\def\faImage{\faicon{image}}\expandafter\def\csname faicon@image\endcsname{\faicon{picture-o}}
\def\faInstitution{\faicon{institution}}\expandafter\def\csname faicon@institution\endcsname{\faicon{university}}
\def\faFileMovieO{\faicon{file-movie-o}}\expandafter\def\csname faicon@file-movie-o\endcsname{\faicon{file-video-o}}
\def\faPhoto{\faicon{photo}}\expandafter\def\csname faicon@photo\endcsname{\faicon{picture-o}}
\def\faFileSoundO{\faicon{file-sound-o}}\expandafter\def\csname faicon@file-sound-o\endcsname{\faicon{file-audio-o}}
\def\faMortarBoard{\faicon{mortar-board}}\expandafter\def\csname faicon@mortar-board\endcsname{\faicon{graduation-cap}}
\def\faGittip{\faicon{gittip}}\expandafter\def\csname faicon@gittip\endcsname{\faicon{gratipay}}
\def\faHourglass2{\faicon{hourglass-2}}\expandafter\def\csname faicon@hourglass-2\endcsname{\faicon{hourglass-half}}
\def\faSupport{\faicon{support}}\expandafter\def\csname faicon@support\endcsname{\faicon{life-ring}}
\def\faEdit{\faicon{edit}}\expandafter\def\csname faicon@edit\endcsname{\faicon{pencil-square-o}}
\def\faHotel{\faicon{hotel}}\expandafter\def\csname faicon@hotel\endcsname{\faicon{bed}}
\def\faSoccerBallO{\faicon{soccer-ball-o}}\expandafter\def\csname faicon@soccer-ball-o\endcsname{\faicon{futbol-o}}
\def\faFilePictureO{\faicon{file-picture-o}}\expandafter\def\csname faicon@file-picture-o\endcsname{\faicon{file-image-o}}
\def\faClose{\faicon{close}}\expandafter\def\csname faicon@close\endcsname{\faicon{times}}
\def\faYcSquare{\faicon{yc-square}}\expandafter\def\csname faicon@yc-square\endcsname{\faicon{hacker-news}}
\def\faShekel{\faicon{shekel}}\expandafter\def\csname faicon@shekel\endcsname{\faicon{ils}}
\def\faDollar{\faicon{dollar}}\expandafter\def\csname faicon@dollar\endcsname{\faicon{usd}}
\def\faUnsorted{\faicon{unsorted}}\expandafter\def\csname faicon@unsorted\endcsname{\faicon{sort}}
\def\faReorder{\faicon{reorder}}\expandafter\def\csname faicon@reorder\endcsname{\faicon{bars}}
\def\faBattery3{\faicon{battery-3}}\expandafter\def\csname faicon@battery-3\endcsname{\faicon{battery-three-quarters}}
\def\faRupee{\faicon{rupee}}\expandafter\def\csname faicon@rupee\endcsname{\faicon{inr}}
\def\faRouble{\faicon{rouble}}\expandafter\def\csname faicon@rouble\endcsname{\faicon{rub}}
\def\faHourglass1{\faicon{hourglass-1}}\expandafter\def\csname faicon@hourglass-1\endcsname{\faicon{hourglass-start}}
\def\faAslInterpreting{\faicon{asl-interpreting}}\expandafter\def\csname faicon@asl-interpreting\endcsname{\faicon{american-sign-language-interpreting}}
\def\faTv{\faicon{tv}}\expandafter\def\csname faicon@tv\endcsname{\faicon{television}}
\def\faSave{\faicon{save}}\expandafter\def\csname faicon@save\endcsname{\faicon{floppy-o}}
\def\faToggleRight{\faicon{toggle-right}}\expandafter\def\csname faicon@toggle-right\endcsname{\faicon{caret-square-o-right}}
\def\faDedent{\faicon{dedent}}\expandafter\def\csname faicon@dedent\endcsname{\faicon{outdent}}
\def\faGear{\faicon{gear}}\expandafter\def\csname faicon@gear\endcsname{\faicon{cog}}
\def\faLegal{\faicon{legal}}\expandafter\def\csname faicon@legal\endcsname{\faicon{gavel}}
\def\faWechat{\faicon{wechat}}\expandafter\def\csname faicon@wechat\endcsname{\faicon{weixin}}
\def\faFacebookF{\faicon{facebook-f}}\expandafter\def\csname faicon@facebook-f\endcsname{\faicon{facebook}}
\def\faFeed{\faicon{feed}}\expandafter\def\csname faicon@feed\endcsname{\faicon{rss}}
\def\faBank{\faicon{bank}}\expandafter\def\csname faicon@bank\endcsname{\faicon{university}}
\def\faTurkishLira{\faicon{turkish-lira}}\expandafter\def\csname faicon@turkish-lira\endcsname{\faicon{try}}
\def\faUnlink{\faicon{unlink}}\expandafter\def\csname faicon@unlink\endcsname{\faicon{chain-broken}}
\def\faChain{\faicon{chain}}\expandafter\def\csname faicon@chain\endcsname{\faicon{link}}
\def\faGears{\faicon{gears}}\expandafter\def\csname faicon@gears\endcsname{\faicon{cogs}}
\def\faRmb{\faicon{rmb}}\expandafter\def\csname faicon@rmb\endcsname{\faicon{jpy}}
\def\faBattery1{\faicon{battery-1}}\expandafter\def\csname faicon@battery-1\endcsname{\faicon{battery-quarter}}
\def\faLifeBouy{\faicon{life-bouy}}\expandafter\def\csname faicon@life-bouy\endcsname{\faicon{life-ring}}
\def\faYen{\faicon{yen}}\expandafter\def\csname faicon@yen\endcsname{\faicon{jpy}}
\def\faBattery4{\faicon{battery-4}}\expandafter\def\csname faicon@battery-4\endcsname{\faicon{battery-full}}
\def\faBattery0{\faicon{battery-0}}\expandafter\def\csname faicon@battery-0\endcsname{\faicon{battery-empty}}
\def\faHandGrabO{\faicon{hand-grab-o}}\expandafter\def\csname faicon@hand-grab-o\endcsname{\faicon{hand-rock-o}}
\def\faMailReplyAll{\faicon{mail-reply-all}}\expandafter\def\csname faicon@mail-reply-all\endcsname{\faicon{reply-all}}
\def\faMobilePhone{\faicon{mobile-phone}}\expandafter\def\csname faicon@mobile-phone\endcsname{\faicon{mobile}}
\def\faRotateLeft{\faicon{rotate-left}}\expandafter\def\csname faicon@rotate-left\endcsname{\faicon{undo}}
\def\faEuro{\faicon{euro}}\expandafter\def\csname faicon@euro\endcsname{\faicon{eur}}
\def\faRuble{\faicon{ruble}}\expandafter\def\csname faicon@ruble\endcsname{\faicon{rub}}
\def\faRa{\faicon{ra}}\expandafter\def\csname faicon@ra\endcsname{\faicon{rebel}}
\def\faStarHalfFull{\faicon{star-half-full}}\expandafter\def\csname faicon@star-half-full\endcsname{\faicon{star-half-o}}
\def\faSortUp{\faicon{sort-up}}\expandafter\def\csname faicon@sort-up\endcsname{\faicon{sort-asc}}
\def\faMailForward{\faicon{mail-forward}}\expandafter\def\csname faicon@mail-forward\endcsname{\faicon{share}}
\def\faSigning{\faicon{signing}}\expandafter\def\csname faicon@signing\endcsname{\faicon{sign-language}}
\def\faFlash{\faicon{flash}}\expandafter\def\csname faicon@flash\endcsname{\faicon{bolt}}
\def\faLifeSaver{\faicon{life-saver}}\expandafter\def\csname faicon@life-saver\endcsname{\faicon{life-ring}}
\def\faFilePhotoO{\faicon{file-photo-o}}\expandafter\def\csname faicon@file-photo-o\endcsname{\faicon{file-image-o}}
\def\faDeafness{\faicon{deafness}}\expandafter\def\csname faicon@deafness\endcsname{\faicon{deaf}}
\def\faBarChartO{\faicon{bar-chart-o}}\expandafter\def\csname faicon@bar-chart-o\endcsname{\faicon{bar-chart}}
\def\faSendO{\faicon{send-o}}\expandafter\def\csname faicon@send-o\endcsname{\faicon{paper-plane-o}}
\def\faNavicon{\faicon{navicon}}\expandafter\def\csname faicon@navicon\endcsname{\faicon{bars}}
\def\faRemove{\faicon{remove}}\expandafter\def\csname faicon@remove\endcsname{\faicon{times}}


==> fontawesomesymbols-pdftex.tex <==
%% start of file `fontawesomesymbols-pdftex.tex'.
\expandafter\def\csname faicon@info\endcsname{{\FAone\symbol{0}}}
\expandafter\def\csname faicon@eraser\endcsname{{\FAone\symbol{1}}}
\expandafter\def\csname faicon@rss-square\endcsname{{\FAone\symbol{2}}}
\expandafter\def\csname faicon@external-link-square\endcsname{{\FAone\symbol{3}}}
\expandafter\def\csname faicon@caret-square-o-right\endcsname{{\FAone\symbol{4}}}
\expandafter\def\csname faicon@sort-alpha-desc\endcsname{{\FAone\symbol{5}}}
\expandafter\def\csname faicon@thumbs-up\endcsname{{\FAone\symbol{6}}}
\expandafter\def\csname faicon@thumbs-down\endcsname{{\FAone\symbol{7}}}
\expandafter\def\csname faicon@moon-o\endcsname{{\FAone\symbol{8}}}
\expandafter\def\csname faicon@pagelines\endcsname{{\FAone\symbol{9}}}
\expandafter\def\csname faicon@arrow-circle-o-right\endcsname{{\FAone\symbol{10}}}
\expandafter\def\csname faicon@caret-square-o-left\endcsname{{\FAone\symbol{11}}}
\expandafter\def\csname faicon@wheelchair\endcsname{{\FAone\symbol{12}}}
\expandafter\def\csname faicon@try\endcsname{{\FAone\symbol{13}}}
\expandafter\def\csname faicon@space-shuttle\endcsname{{\FAone\symbol{14}}}
\expandafter\def\csname faicon@slack\endcsname{{\FAone\symbol{15}}}
\expandafter\def\csname faicon@envelope-square\endcsname{{\FAone\symbol{16}}}
\expandafter\def\csname faicon@wordpress\endcsname{{\FAone\symbol{17}}}
\expandafter\def\csname faicon@openid\endcsname{{\FAone\symbol{18}}}
\expandafter\def\csname faicon@university\endcsname{{\FAone\symbol{19}}}
\expandafter\def\csname faicon@graduation-cap\endcsname{{\FAone\symbol{20}}}
\expandafter\def\csname faicon@yahoo\endcsname{{\FAone\symbol{21}}}
\expandafter\def\csname faicon@reddit-square\endcsname{{\FAone\symbol{22}}}
\expandafter\def\csname faicon@stumbleupon-circle\endcsname{{\FAone\symbol{23}}}
\expandafter\def\csname faicon@delicious\endcsname{{\FAone\symbol{24}}}
\expandafter\def\csname faicon@digg\endcsname{{\FAone\symbol{25}}}
\expandafter\def\csname faicon@pied-piper-pp\endcsname{{\FAone\symbol{26}}}
\expandafter\def\csname faicon@pied-piper-alt\endcsname{{\FAone\symbol{27}}}
\expandafter\def\csname faicon@drupal\endcsname{{\FAone\symbol{28}}}
\expandafter\def\csname faicon@joomla\endcsname{{\FAone\symbol{29}}}
\expandafter\def\csname faicon@fax\endcsname{{\FAone\symbol{30}}}
\expandafter\def\csname faicon@building\endcsname{{\FAone\symbol{31}}}
\expandafter\def\csname faicon@child\endcsname{{\FAone\symbol{32}}}
\expandafter\def\csname faicon@spoon\endcsname{{\FAone\symbol{33}}}
\expandafter\def\csname faicon@cube\endcsname{{\FAone\symbol{34}}}
\expandafter\def\csname faicon@cubes\endcsname{{\FAone\symbol{35}}}
\expandafter\def\csname faicon@behance\endcsname{{\FAone\symbol{36}}}
\expandafter\def\csname faicon@behance-square\endcsname{{\FAone\symbol{37}}}
\expandafter\def\csname faicon@steam\endcsname{{\FAone\symbol{38}}}
\expandafter\def\csname faicon@steam-square\endcsname{{\FAone\symbol{39}}}
\expandafter\def\csname faicon@recycle\endcsname{{\FAone\symbol{40}}}
\expandafter\def\csname faicon@car\endcsname{{\FAone\symbol{41}}}
\expandafter\def\csname faicon@taxi\endcsname{{\FAone\symbol{42}}}
\expandafter\def\csname faicon@tree\endcsname{{\FAone\symbol{43}}}
\expandafter\def\csname faicon@spotify\endcsname{{\FAone\symbol{44}}}
\expandafter\def\csname faicon@deviantart\endcsname{{\FAone\symbol{45}}}
\expandafter\def\csname faicon@soundcloud\endcsname{{\FAone\symbol{46}}}
\expandafter\def\csname faicon@file-word-o\endcsname{{\FAone\symbol{47}}}
\expandafter\def\csname faicon@file-excel-o\endcsname{{\FAone\symbol{48}}}
\expandafter\def\csname faicon@file-powerpoint-o\endcsname{{\FAone\symbol{49}}}
\expandafter\def\csname faicon@file-image-o\endcsname{{\FAone\symbol{50}}}
\expandafter\def\csname faicon@file-archive-o\endcsname{{\FAone\symbol{51}}}
\expandafter\def\csname faicon@file-audio-o\endcsname{{\FAone\symbol{52}}}
\expandafter\def\csname faicon@file-video-o\endcsname{{\FAone\symbol{53}}}
\expandafter\def\csname faicon@file-code-o\endcsname{{\FAone\symbol{54}}}
\expandafter\def\csname faicon@vine\endcsname{{\FAone\symbol{55}}}
\expandafter\def\csname faicon@codepen\endcsname{{\FAone\symbol{56}}}
\expandafter\def\csname faicon@jsfiddle\endcsname{{\FAone\symbol{57}}}
\expandafter\def\csname faicon@life-ring\endcsname{{\FAone\symbol{58}}}
\expandafter\def\csname faicon@circle-o-notch\endcsname{{\FAone\symbol{59}}}
\expandafter\def\csname faicon@git\endcsname{{\FAone\symbol{60}}}
\expandafter\def\csname faicon@hacker-news\endcsname{{\FAone\symbol{61}}}
\expandafter\def\csname faicon@paper-plane\endcsname{{\FAone\symbol{62}}}
\expandafter\def\csname faicon@paper-plane-o\endcsname{{\FAone\symbol{63}}}
\expandafter\def\csname faicon@history\endcsname{{\FAone\symbol{64}}}
\expandafter\def\csname faicon@circle-thin\endcsname{{\FAone\symbol{65}}}
\expandafter\def\csname faicon@header\endcsname{{\FAone\symbol{66}}}
\expandafter\def\csname faicon@paragraph\endcsname{{\FAone\symbol{67}}}
\expandafter\def\csname faicon@sliders\endcsname{{\FAone\symbol{68}}}
\expandafter\def\csname faicon@share-alt-square\endcsname{{\FAone\symbol{69}}}
\expandafter\def\csname faicon@bomb\endcsname{{\FAone\symbol{70}}}
\expandafter\def\csname faicon@futbol-o\endcsname{{\FAone\symbol{71}}}
\expandafter\def\csname faicon@tty\endcsname{{\FAone\symbol{72}}}
\expandafter\def\csname faicon@binoculars\endcsname{{\FAone\symbol{73}}}
\expandafter\def\csname faicon@plug\endcsname{{\FAone\symbol{74}}}
\expandafter\def\csname faicon@slideshare\endcsname{{\FAone\symbol{75}}}
\expandafter\def\csname faicon@twitch\endcsname{{\FAone\symbol{76}}}
\expandafter\def\csname faicon@yelp\endcsname{{\FAone\symbol{77}}}
\expandafter\def\csname faicon@newspaper-o\endcsname{{\FAone\symbol{78}}}
\expandafter\def\csname faicon@wifi\endcsname{{\FAone\symbol{79}}}
\expandafter\def\csname faicon@calculator\endcsname{{\FAone\symbol{80}}}
\expandafter\def\csname faicon@paypal\endcsname{{\FAone\symbol{81}}}
\expandafter\def\csname faicon@google-wallet\endcsname{{\FAone\symbol{82}}}
\expandafter\def\csname faicon@cc-mastercard\endcsname{{\FAone\symbol{83}}}
\expandafter\def\csname faicon@cc-discover\endcsname{{\FAone\symbol{84}}}
\expandafter\def\csname faicon@cc-paypal\endcsname{{\FAone\symbol{85}}}
\expandafter\def\csname faicon@cc-stripe\endcsname{{\FAone\symbol{86}}}
\expandafter\def\csname faicon@bell-slash\endcsname{{\FAone\symbol{87}}}
\expandafter\def\csname faicon@bell-slash-o\endcsname{{\FAone\symbol{88}}}
\expandafter\def\csname faicon@trash\endcsname{{\FAone\symbol{89}}}
\expandafter\def\csname faicon@copyright\endcsname{{\FAone\symbol{90}}}
\expandafter\def\csname faicon@at\endcsname{{\FAone\symbol{91}}}
\expandafter\def\csname faicon@eyedropper\endcsname{{\FAone\symbol{92}}}
\expandafter\def\csname faicon@birthday-cake\endcsname{{\FAone\symbol{93}}}
\expandafter\def\csname faicon@area-chart\endcsname{{\FAone\symbol{94}}}
\expandafter\def\csname faicon@pie-chart\endcsname{{\FAone\symbol{95}}}
\expandafter\def\csname faicon@line-chart\endcsname{{\FAone\symbol{96}}}
\expandafter\def\csname faicon@lastfm\endcsname{{\FAone\symbol{97}}}
\expandafter\def\csname faicon@lastfm-square\endcsname{{\FAone\symbol{98}}}
\expandafter\def\csname faicon@toggle-off\endcsname{{\FAone\symbol{99}}}
\expandafter\def\csname faicon@toggle-on\endcsname{{\FAone\symbol{100}}}
\expandafter\def\csname faicon@bicycle\endcsname{{\FAone\symbol{101}}}
\expandafter\def\csname faicon@bus\endcsname{{\FAone\symbol{102}}}
\expandafter\def\csname faicon@ioxhost\endcsname{{\FAone\symbol{103}}}
\expandafter\def\csname faicon@angellist\endcsname{{\FAone\symbol{104}}}
\expandafter\def\csname faicon@cc\endcsname{{\FAone\symbol{105}}}
\expandafter\def\csname faicon@ils\endcsname{{\FAone\symbol{106}}}
\expandafter\def\csname faicon@meanpath\endcsname{{\FAone\symbol{107}}}
\expandafter\def\csname faicon@buysellads\endcsname{{\FAone\symbol{108}}}
\expandafter\def\csname faicon@connectdevelop\endcsname{{\FAone\symbol{109}}}
\expandafter\def\csname faicon@forumbee\endcsname{{\FAone\symbol{110}}}
\expandafter\def\csname faicon@sellsy\endcsname{{\FAone\symbol{111}}}
\expandafter\def\csname faicon@shirtsinbulk\endcsname{{\FAone\symbol{112}}}
\expandafter\def\csname faicon@simplybuilt\endcsname{{\FAone\symbol{113}}}
\expandafter\def\csname faicon@skyatlas\endcsname{{\FAone\symbol{114}}}
\expandafter\def\csname faicon@cart-plus\endcsname{{\FAone\symbol{115}}}
\expandafter\def\csname faicon@cart-arrow-down\endcsname{{\FAone\symbol{116}}}
\expandafter\def\csname faicon@diamond\endcsname{{\FAone\symbol{117}}}
\expandafter\def\csname faicon@ship\endcsname{{\FAone\symbol{118}}}
\expandafter\def\csname faicon@user-secret\endcsname{{\FAone\symbol{119}}}
\expandafter\def\csname faicon@motorcycle\endcsname{{\FAone\symbol{120}}}
\expandafter\def\csname faicon@street-view\endcsname{{\FAone\symbol{121}}}
\expandafter\def\csname faicon@heartbeat\endcsname{{\FAone\symbol{122}}}
\expandafter\def\csname faicon@mars\endcsname{{\FAone\symbol{123}}}
\expandafter\def\csname faicon@mercury\endcsname{{\FAone\symbol{124}}}
\expandafter\def\csname faicon@transgender\endcsname{{\FAone\symbol{125}}}
\expandafter\def\csname faicon@transgender-alt\endcsname{{\FAone\symbol{126}}}
\expandafter\def\csname faicon@venus-double\endcsname{{\FAone\symbol{127}}}
\expandafter\def\csname faicon@mars-double\endcsname{{\FAone\symbol{128}}}
\expandafter\def\csname faicon@venus-mars\endcsname{{\FAone\symbol{129}}}
\expandafter\def\csname faicon@mars-stroke\endcsname{{\FAone\symbol{130}}}
\expandafter\def\csname faicon@mars-stroke-v\endcsname{{\FAone\symbol{131}}}
\expandafter\def\csname faicon@mars-stroke-h\endcsname{{\FAone\symbol{132}}}
\expandafter\def\csname faicon@neuter\endcsname{{\FAone\symbol{133}}}
\expandafter\def\csname faicon@genderless\endcsname{{\FAone\symbol{134}}}
\expandafter\def\csname faicon@facebook-official\endcsname{{\FAone\symbol{135}}}
\expandafter\def\csname faicon@pinterest-p\endcsname{{\FAone\symbol{136}}}
\expandafter\def\csname faicon@whatsapp\endcsname{{\FAone\symbol{137}}}
\expandafter\def\csname faicon@server\endcsname{{\FAone\symbol{138}}}
\expandafter\def\csname faicon@user-plus\endcsname{{\FAone\symbol{139}}}
\expandafter\def\csname faicon@user-times\endcsname{{\FAone\symbol{140}}}
\expandafter\def\csname faicon@bed\endcsname{{\FAone\symbol{141}}}
\expandafter\def\csname faicon@viacoin\endcsname{{\FAone\symbol{142}}}
\expandafter\def\csname faicon@train\endcsname{{\FAone\symbol{143}}}
\expandafter\def\csname faicon@subway\endcsname{{\FAone\symbol{144}}}
\expandafter\def\csname faicon@medium\endcsname{{\FAone\symbol{145}}}
\expandafter\def\csname faicon@y-combinator\endcsname{{\FAone\symbol{146}}}
\expandafter\def\csname faicon@optin-monster\endcsname{{\FAone\symbol{147}}}
\expandafter\def\csname faicon@opencart\endcsname{{\FAone\symbol{148}}}
\expandafter\def\csname faicon@expeditedssl\endcsname{{\FAone\symbol{149}}}
\expandafter\def\csname faicon@battery-full\endcsname{{\FAone\symbol{150}}}
\expandafter\def\csname faicon@battery-three-quarters\endcsname{{\FAone\symbol{151}}}
\expandafter\def\csname faicon@battery-half\endcsname{{\FAone\symbol{152}}}
\expandafter\def\csname faicon@battery-quarter\endcsname{{\FAone\symbol{153}}}
\expandafter\def\csname faicon@battery-empty\endcsname{{\FAone\symbol{154}}}
\expandafter\def\csname faicon@mouse-pointer\endcsname{{\FAone\symbol{155}}}
\expandafter\def\csname faicon@i-cursor\endcsname{{\FAone\symbol{156}}}
\expandafter\def\csname faicon@object-group\endcsname{{\FAone\symbol{157}}}
\expandafter\def\csname faicon@object-ungroup\endcsname{{\FAone\symbol{158}}}
\expandafter\def\csname faicon@sticky-note\endcsname{{\FAone\symbol{159}}}
\expandafter\def\csname faicon@sticky-note-o\endcsname{{\FAone\symbol{160}}}
\expandafter\def\csname faicon@cc-jcb\endcsname{{\FAone\symbol{161}}}
\expandafter\def\csname faicon@cc-diners-club\endcsname{{\FAone\symbol{162}}}
\expandafter\def\csname faicon@clone\endcsname{{\FAone\symbol{163}}}
\expandafter\def\csname faicon@balance-scale\endcsname{{\FAone\symbol{164}}}
\expandafter\def\csname faicon@hourglass-o\endcsname{{\FAone\symbol{165}}}
\expandafter\def\csname faicon@hourglass-start\endcsname{{\FAone\symbol{166}}}
\expandafter\def\csname faicon@hourglass-half\endcsname{{\FAone\symbol{167}}}
\expandafter\def\csname faicon@hourglass-end\endcsname{{\FAone\symbol{168}}}
\expandafter\def\csname faicon@hourglass\endcsname{{\FAone\symbol{169}}}
\expandafter\def\csname faicon@hand-rock-o\endcsname{{\FAone\symbol{170}}}
\expandafter\def\csname faicon@hand-paper-o\endcsname{{\FAone\symbol{171}}}
\expandafter\def\csname faicon@hand-scissors-o\endcsname{{\FAone\symbol{172}}}
\expandafter\def\csname faicon@hand-lizard-o\endcsname{{\FAone\symbol{173}}}
\expandafter\def\csname faicon@hand-spock-o\endcsname{{\FAone\symbol{174}}}
\expandafter\def\csname faicon@hand-pointer-o\endcsname{{\FAone\symbol{175}}}
\expandafter\def\csname faicon@hand-peace-o\endcsname{{\FAone\symbol{176}}}
\expandafter\def\csname faicon@trademark\endcsname{{\FAone\symbol{177}}}
\expandafter\def\csname faicon@registered\endcsname{{\FAone\symbol{178}}}
\expandafter\def\csname faicon@creative-commons\endcsname{{\FAone\symbol{179}}}
\expandafter\def\csname faicon@tripadvisor\endcsname{{\FAone\symbol{180}}}
\expandafter\def\csname faicon@odnoklassniki-square\endcsname{{\FAone\symbol{181}}}
\expandafter\def\csname faicon@get-pocket\endcsname{{\FAone\symbol{182}}}
\expandafter\def\csname faicon@wikipedia-w\endcsname{{\FAone\symbol{183}}}
\expandafter\def\csname faicon@safari\endcsname{{\FAone\symbol{184}}}
\expandafter\def\csname faicon@chrome\endcsname{{\FAone\symbol{185}}}
\expandafter\def\csname faicon@firefox\endcsname{{\FAone\symbol{186}}}
\expandafter\def\csname faicon@opera\endcsname{{\FAone\symbol{187}}}
\expandafter\def\csname faicon@internet-explorer\endcsname{{\FAone\symbol{188}}}
\expandafter\def\csname faicon@television\endcsname{{\FAone\symbol{189}}}
\expandafter\def\csname faicon@contao\endcsname{{\FAone\symbol{190}}}
\expandafter\def\csname faicon@500px\endcsname{{\FAone\symbol{191}}}
\expandafter\def\csname faicon@amazon\endcsname{{\FAone\symbol{192}}}
\expandafter\def\csname faicon@calendar-plus-o\endcsname{{\FAone\symbol{193}}}
\expandafter\def\csname faicon@calendar-minus-o\endcsname{{\FAone\symbol{194}}}
\expandafter\def\csname faicon@calendar-times-o\endcsname{{\FAone\symbol{195}}}
\expandafter\def\csname faicon@calendar-check-o\endcsname{{\FAone\symbol{196}}}
\expandafter\def\csname faicon@industry\endcsname{{\FAone\symbol{197}}}
\expandafter\def\csname faicon@map-pin\endcsname{{\FAone\symbol{198}}}
\expandafter\def\csname faicon@map-signs\endcsname{{\FAone\symbol{199}}}
\expandafter\def\csname faicon@map-o\endcsname{{\FAone\symbol{200}}}
\expandafter\def\csname faicon@map\endcsname{{\FAone\symbol{201}}}
\expandafter\def\csname faicon@commenting\endcsname{{\FAone\symbol{202}}}
\expandafter\def\csname faicon@commenting-o\endcsname{{\FAone\symbol{203}}}
\expandafter\def\csname faicon@houzz\endcsname{{\FAone\symbol{204}}}
\expandafter\def\csname faicon@vimeo\endcsname{{\FAone\symbol{205}}}
\expandafter\def\csname faicon@edge\endcsname{{\FAone\symbol{206}}}
\expandafter\def\csname faicon@credit-card-alt\endcsname{{\FAone\symbol{207}}}
\expandafter\def\csname faicon@codiepie\endcsname{{\FAone\symbol{208}}}
\expandafter\def\csname faicon@usb\endcsname{{\FAone\symbol{209}}}
\expandafter\def\csname faicon@product-hunt\endcsname{{\FAone\symbol{210}}}
\expandafter\def\csname faicon@mixcloud\endcsname{{\FAone\symbol{211}}}
\expandafter\def\csname faicon@scribd\endcsname{{\FAone\symbol{212}}}
\expandafter\def\csname faicon@pause-circle\endcsname{{\FAone\symbol{213}}}
\expandafter\def\csname faicon@pause-circle-o\endcsname{{\FAone\symbol{214}}}
\expandafter\def\csname faicon@stop-circle\endcsname{{\FAone\symbol{215}}}
\expandafter\def\csname faicon@stop-circle-o\endcsname{{\FAone\symbol{216}}}
\expandafter\def\csname faicon@shopping-bag\endcsname{{\FAone\symbol{217}}}
\expandafter\def\csname faicon@shopping-basket\endcsname{{\FAone\symbol{218}}}
\expandafter\def\csname faicon@hashtag\endcsname{{\FAone\symbol{219}}}
\expandafter\def\csname faicon@bluetooth\endcsname{{\FAone\symbol{220}}}
\expandafter\def\csname faicon@bluetooth-b\endcsname{{\FAone\symbol{221}}}
\expandafter\def\csname faicon@percent\endcsname{{\FAone\symbol{222}}}
\expandafter\def\csname faicon@gitlab\endcsname{{\FAone\symbol{223}}}
\expandafter\def\csname faicon@wpbeginner\endcsname{{\FAone\symbol{224}}}
\expandafter\def\csname faicon@wpforms\endcsname{{\FAone\symbol{225}}}
\expandafter\def\csname faicon@envira\endcsname{{\FAone\symbol{226}}}
\expandafter\def\csname faicon@universal-access\endcsname{{\FAone\symbol{227}}}
\expandafter\def\csname faicon@wheelchair-alt\endcsname{{\FAone\symbol{228}}}
\expandafter\def\csname faicon@question-circle-o\endcsname{{\FAone\symbol{229}}}
\expandafter\def\csname faicon@blind\endcsname{{\FAone\symbol{230}}}
\expandafter\def\csname faicon@audio-description\endcsname{{\FAone\symbol{231}}}
\expandafter\def\csname faicon@adjust\endcsname{{\FAone\symbol{232}}}
\expandafter\def\csname faicon@adn\endcsname{{\FAone\symbol{233}}}
\expandafter\def\csname faicon@align-center\endcsname{{\FAone\symbol{234}}}
\expandafter\def\csname faicon@align-justify\endcsname{{\FAone\symbol{235}}}
\expandafter\def\csname faicon@align-left\endcsname{{\FAone\symbol{236}}}
\expandafter\def\csname faicon@align-right\endcsname{{\FAone\symbol{237}}}
\expandafter\def\csname faicon@ambulance\endcsname{{\FAone\symbol{238}}}
\expandafter\def\csname faicon@anchor\endcsname{{\FAone\symbol{239}}}
\expandafter\def\csname faicon@android\endcsname{{\FAone\symbol{240}}}
\expandafter\def\csname faicon@angle-down\endcsname{{\FAone\symbol{241}}}
\expandafter\def\csname faicon@angle-left\endcsname{{\FAone\symbol{242}}}
\expandafter\def\csname faicon@angle-right\endcsname{{\FAone\symbol{243}}}
\expandafter\def\csname faicon@angle-up\endcsname{{\FAone\symbol{244}}}
\expandafter\def\csname faicon@apple\endcsname{{\FAone\symbol{245}}}
\expandafter\def\csname faicon@archive\endcsname{{\FAone\symbol{246}}}
\expandafter\def\csname faicon@arrow-circle-o-left\endcsname{{\FAone\symbol{247}}}
\expandafter\def\csname faicon@arrow-down\endcsname{{\FAone\symbol{248}}}
\expandafter\def\csname faicon@arrow-left\endcsname{{\FAone\symbol{249}}}
\expandafter\def\csname faicon@arrow-right\endcsname{{\FAone\symbol{250}}}
\expandafter\def\csname faicon@arrow-up\endcsname{{\FAone\symbol{251}}}
\expandafter\def\csname faicon@asterisk\endcsname{{\FAone\symbol{252}}}
\expandafter\def\csname faicon@backward\endcsname{{\FAone\symbol{253}}}
\expandafter\def\csname faicon@ban\endcsname{{\FAone\symbol{254}}}
\expandafter\def\csname faicon@bar-chart\endcsname{{\FAone\symbol{255}}}
\expandafter\def\csname faicon@barcode\endcsname{{\FAtwo\symbol{0}}}
\expandafter\def\csname faicon@flask\endcsname{{\FAtwo\symbol{1}}}
\expandafter\def\csname faicon@beer\endcsname{{\FAtwo\symbol{2}}}
\expandafter\def\csname faicon@bell-o\endcsname{{\FAtwo\symbol{3}}}
\expandafter\def\csname faicon@bell\endcsname{{\FAtwo\symbol{4}}}
\expandafter\def\csname faicon@bitbucket-square\endcsname{{\FAtwo\symbol{5}}}
\expandafter\def\csname faicon@bold\endcsname{{\FAtwo\symbol{6}}}
\expandafter\def\csname faicon@bolt\endcsname{{\FAtwo\symbol{7}}}
\expandafter\def\csname faicon@book\endcsname{{\FAtwo\symbol{8}}}
\expandafter\def\csname faicon@bookmark\endcsname{{\FAtwo\symbol{9}}}
\expandafter\def\csname faicon@bookmark-o\endcsname{{\FAtwo\symbol{10}}}
\expandafter\def\csname faicon@briefcase\endcsname{{\FAtwo\symbol{11}}}
\expandafter\def\csname faicon@btc\endcsname{{\FAtwo\symbol{12}}}
\expandafter\def\csname faicon@bug\endcsname{{\FAtwo\symbol{13}}}
\expandafter\def\csname faicon@building-o\endcsname{{\FAtwo\symbol{14}}}
\expandafter\def\csname faicon@bullhorn\endcsname{{\FAtwo\symbol{15}}}
\expandafter\def\csname faicon@bullseye\endcsname{{\FAtwo\symbol{16}}}
\expandafter\def\csname faicon@calendar\endcsname{{\FAtwo\symbol{17}}}
\expandafter\def\csname faicon@calendar-o\endcsname{{\FAtwo\symbol{18}}}
\expandafter\def\csname faicon@camera\endcsname{{\FAtwo\symbol{19}}}
\expandafter\def\csname faicon@camera-retro\endcsname{{\FAtwo\symbol{20}}}
\expandafter\def\csname faicon@caret-down\endcsname{{\FAtwo\symbol{21}}}
\expandafter\def\csname faicon@caret-left\endcsname{{\FAtwo\symbol{22}}}
\expandafter\def\csname faicon@caret-right\endcsname{{\FAtwo\symbol{23}}}
\expandafter\def\csname faicon@caret-up\endcsname{{\FAtwo\symbol{24}}}
\expandafter\def\csname faicon@certificate\endcsname{{\FAtwo\symbol{25}}}
\expandafter\def\csname faicon@check-square-o\endcsname{{\FAtwo\symbol{26}}}
\expandafter\def\csname faicon@square-o\endcsname{{\FAtwo\symbol{27}}}
\expandafter\def\csname faicon@minus-square-o\endcsname{{\FAtwo\symbol{28}}}
\expandafter\def\csname faicon@check-square\endcsname{{\FAtwo\symbol{29}}}
\expandafter\def\csname faicon@chevron-down\endcsname{{\FAtwo\symbol{30}}}
\expandafter\def\csname faicon@chevron-left\endcsname{{\FAtwo\symbol{31}}}
\expandafter\def\csname faicon@chevron-right\endcsname{{\FAtwo\symbol{32}}}
\expandafter\def\csname faicon@chevron-circle-down\endcsname{{\FAtwo\symbol{33}}}
\expandafter\def\csname faicon@chevron-circle-left\endcsname{{\FAtwo\symbol{34}}}
\expandafter\def\csname faicon@chevron-circle-right\endcsname{{\FAtwo\symbol{35}}}
\expandafter\def\csname faicon@chevron-circle-up\endcsname{{\FAtwo\symbol{36}}}
\expandafter\def\csname faicon@chevron-up\endcsname{{\FAtwo\symbol{37}}}
\expandafter\def\csname faicon@circle\endcsname{{\FAtwo\symbol{38}}}
\expandafter\def\csname faicon@arrow-circle-down\endcsname{{\FAtwo\symbol{39}}}
\expandafter\def\csname faicon@arrow-circle-left\endcsname{{\FAtwo\symbol{40}}}
\expandafter\def\csname faicon@arrow-circle-right\endcsname{{\FAtwo\symbol{41}}}
\expandafter\def\csname faicon@arrow-circle-up\endcsname{{\FAtwo\symbol{42}}}
\expandafter\def\csname faicon@circle-o\endcsname{{\FAtwo\symbol{43}}}
\expandafter\def\csname faicon@cloud\endcsname{{\FAtwo\symbol{44}}}
\expandafter\def\csname faicon@cloud-download\endcsname{{\FAtwo\symbol{45}}}
\expandafter\def\csname faicon@cloud-upload\endcsname{{\FAtwo\symbol{46}}}
\expandafter\def\csname faicon@code\endcsname{{\FAtwo\symbol{47}}}
\expandafter\def\csname faicon@code-fork\endcsname{{\FAtwo\symbol{48}}}
\expandafter\def\csname faicon@coffee\endcsname{{\FAtwo\symbol{49}}}
\expandafter\def\csname faicon@cog\endcsname{{\FAtwo\symbol{50}}}
\expandafter\def\csname faicon@cogs\endcsname{{\FAtwo\symbol{51}}}
\expandafter\def\csname faicon@caret-square-o-down\endcsname{{\FAtwo\symbol{52}}}
\expandafter\def\csname faicon@caret-square-o-up\endcsname{{\FAtwo\symbol{53}}}
\expandafter\def\csname faicon@columns\endcsname{{\FAtwo\symbol{54}}}
\expandafter\def\csname faicon@comment\endcsname{{\FAtwo\symbol{55}}}
\expandafter\def\csname faicon@comment-o\endcsname{{\FAtwo\symbol{56}}}
\expandafter\def\csname faicon@comments\endcsname{{\FAtwo\symbol{57}}}
\expandafter\def\csname faicon@comments-o\endcsname{{\FAtwo\symbol{58}}}
\expandafter\def\csname faicon@compass\endcsname{{\FAtwo\symbol{59}}}
\expandafter\def\csname faicon@files-o\endcsname{{\FAtwo\symbol{60}}}
\expandafter\def\csname faicon@credit-card\endcsname{{\FAtwo\symbol{61}}}
\expandafter\def\csname faicon@crop\endcsname{{\FAtwo\symbol{62}}}
\expandafter\def\csname faicon@css3\endcsname{{\FAtwo\symbol{63}}}
\expandafter\def\csname faicon@scissors\endcsname{{\FAtwo\symbol{64}}}
\expandafter\def\csname faicon@tachometer\endcsname{{\FAtwo\symbol{65}}}
\expandafter\def\csname faicon@desktop\endcsname{{\FAtwo\symbol{66}}}
\expandafter\def\csname faicon@dot-circle-o\endcsname{{\FAtwo\symbol{67}}}
\expandafter\def\csname faicon@angle-double-down\endcsname{{\FAtwo\symbol{68}}}
\expandafter\def\csname faicon@angle-double-left\endcsname{{\FAtwo\symbol{69}}}
\expandafter\def\csname faicon@angle-double-right\endcsname{{\FAtwo\symbol{70}}}
\expandafter\def\csname faicon@angle-double-up\endcsname{{\FAtwo\symbol{71}}}
\expandafter\def\csname faicon@arrow-circle-o-down\endcsname{{\FAtwo\symbol{72}}}
\expandafter\def\csname faicon@download\endcsname{{\FAtwo\symbol{73}}}
\expandafter\def\csname faicon@dribbble\endcsname{{\FAtwo\symbol{74}}}
\expandafter\def\csname faicon@dropbox\endcsname{{\FAtwo\symbol{75}}}
\expandafter\def\csname faicon@pencil-square-o\endcsname{{\FAtwo\symbol{76}}}
\expandafter\def\csname faicon@pencil-square\endcsname{{\FAtwo\symbol{77}}}
\expandafter\def\csname faicon@eject\endcsname{{\FAtwo\symbol{78}}}
\expandafter\def\csname faicon@ellipsis-h\endcsname{{\FAtwo\symbol{79}}}
\expandafter\def\csname faicon@ellipsis-v\endcsname{{\FAtwo\symbol{80}}}
\expandafter\def\csname faicon@envelope-o\endcsname{{\FAtwo\symbol{81}}}
\expandafter\def\csname faicon@envelope\endcsname{{\FAtwo\symbol{82}}}
\expandafter\def\csname faicon@eur\endcsname{{\FAtwo\symbol{83}}}
\expandafter\def\csname faicon@exchange\endcsname{{\FAtwo\symbol{84}}}
\expandafter\def\csname faicon@exclamation\endcsname{{\FAtwo\symbol{85}}}
\expandafter\def\csname faicon@exclamation-circle\endcsname{{\FAtwo\symbol{86}}}
\expandafter\def\csname faicon@external-link\endcsname{{\FAtwo\symbol{87}}}
\expandafter\def\csname faicon@eye-slash\endcsname{{\FAtwo\symbol{88}}}
\expandafter\def\csname faicon@eye\endcsname{{\FAtwo\symbol{89}}}
\expandafter\def\csname faicon@plus-square\endcsname{{\FAtwo\symbol{90}}}
\expandafter\def\csname faicon@bitbucket\endcsname{{\FAtwo\symbol{91}}}
\expandafter\def\csname faicon@reddit\endcsname{{\FAtwo\symbol{92}}}
\expandafter\def\csname faicon@stumbleupon\endcsname{{\FAtwo\symbol{93}}}
\expandafter\def\csname faicon@language\endcsname{{\FAtwo\symbol{94}}}
\expandafter\def\csname faicon@cc-amex\endcsname{{\FAtwo\symbol{95}}}
\expandafter\def\csname faicon@paint-brush\endcsname{{\FAtwo\symbol{96}}}
\expandafter\def\csname faicon@dashcube\endcsname{{\FAtwo\symbol{97}}}
\expandafter\def\csname faicon@leanpub\endcsname{{\FAtwo\symbol{98}}}
\expandafter\def\csname faicon@gg\endcsname{{\FAtwo\symbol{99}}}
\expandafter\def\csname faicon@gg-circle\endcsname{{\FAtwo\symbol{100}}}
\expandafter\def\csname faicon@odnoklassniki\endcsname{{\FAtwo\symbol{101}}}
\expandafter\def\csname faicon@black-tie\endcsname{{\FAtwo\symbol{102}}}
\expandafter\def\csname faicon@facebook\endcsname{{\FAtwo\symbol{103}}}
\expandafter\def\csname faicon@facebook-square\endcsname{{\FAtwo\symbol{104}}}
\expandafter\def\csname faicon@video-camera\endcsname{{\FAtwo\symbol{105}}}
\expandafter\def\csname faicon@fast-backward\endcsname{{\FAtwo\symbol{106}}}
\expandafter\def\csname faicon@fast-forward\endcsname{{\FAtwo\symbol{107}}}
\expandafter\def\csname faicon@female\endcsname{{\FAtwo\symbol{108}}}
\expandafter\def\csname faicon@fighter-jet\endcsname{{\FAtwo\symbol{109}}}
\expandafter\def\csname faicon@file\endcsname{{\FAtwo\symbol{110}}}
\expandafter\def\csname faicon@file-o\endcsname{{\FAtwo\symbol{111}}}
\expandafter\def\csname faicon@file-text\endcsname{{\FAtwo\symbol{112}}}
\expandafter\def\csname faicon@file-text-o\endcsname{{\FAtwo\symbol{113}}}
\expandafter\def\csname faicon@film\endcsname{{\FAtwo\symbol{114}}}
\expandafter\def\csname faicon@filter\endcsname{{\FAtwo\symbol{115}}}
\expandafter\def\csname faicon@fire\endcsname{{\FAtwo\symbol{116}}}
\expandafter\def\csname faicon@fire-extinguisher\endcsname{{\FAtwo\symbol{117}}}
\expandafter\def\csname faicon@flag\endcsname{{\FAtwo\symbol{118}}}
\expandafter\def\csname faicon@flag-o\endcsname{{\FAtwo\symbol{119}}}
\expandafter\def\csname faicon@flag-checkered\endcsname{{\FAtwo\symbol{120}}}
\expandafter\def\csname faicon@flickr\endcsname{{\FAtwo\symbol{121}}}
\expandafter\def\csname faicon@folder\endcsname{{\FAtwo\symbol{122}}}
\expandafter\def\csname faicon@folder-o\endcsname{{\FAtwo\symbol{123}}}
\expandafter\def\csname faicon@folder-open\endcsname{{\FAtwo\symbol{124}}}
\expandafter\def\csname faicon@folder-open-o\endcsname{{\FAtwo\symbol{125}}}
\expandafter\def\csname faicon@font\endcsname{{\FAtwo\symbol{126}}}
\expandafter\def\csname faicon@cutlery\endcsname{{\FAtwo\symbol{127}}}
\expandafter\def\csname faicon@forward\endcsname{{\FAtwo\symbol{128}}}
\expandafter\def\csname faicon@foursquare\endcsname{{\FAtwo\symbol{129}}}
\expandafter\def\csname faicon@frown-o\endcsname{{\FAtwo\symbol{130}}}
\expandafter\def\csname faicon@arrows-alt\endcsname{{\FAtwo\symbol{131}}}
\expandafter\def\csname faicon@gamepad\endcsname{{\FAtwo\symbol{132}}}
\expandafter\def\csname faicon@gbp\endcsname{{\FAtwo\symbol{133}}}
\expandafter\def\csname faicon@gift\endcsname{{\FAtwo\symbol{134}}}
\expandafter\def\csname faicon@github\endcsname{{\FAtwo\symbol{135}}}
\expandafter\def\csname faicon@github-alt\endcsname{{\FAtwo\symbol{136}}}
\expandafter\def\csname faicon@github-square\endcsname{{\FAtwo\symbol{137}}}
\expandafter\def\csname faicon@gratipay\endcsname{{\FAtwo\symbol{138}}}
\expandafter\def\csname faicon@glass\endcsname{{\FAtwo\symbol{139}}}
\expandafter\def\csname faicon@globe\endcsname{{\FAtwo\symbol{140}}}
\expandafter\def\csname faicon@google-plus\endcsname{{\FAtwo\symbol{141}}}
\expandafter\def\csname faicon@google-plus-square\endcsname{{\FAtwo\symbol{142}}}
\expandafter\def\csname faicon@users\endcsname{{\FAtwo\symbol{143}}}
\expandafter\def\csname faicon@h-square\endcsname{{\FAtwo\symbol{144}}}
\expandafter\def\csname faicon@hand-o-down\endcsname{{\FAtwo\symbol{145}}}
\expandafter\def\csname faicon@hand-o-left\endcsname{{\FAtwo\symbol{146}}}
\expandafter\def\csname faicon@hand-o-right\endcsname{{\FAtwo\symbol{147}}}
\expandafter\def\csname faicon@hand-o-up\endcsname{{\FAtwo\symbol{148}}}
\expandafter\def\csname faicon@hdd-o\endcsname{{\FAtwo\symbol{149}}}
\expandafter\def\csname faicon@headphones\endcsname{{\FAtwo\symbol{150}}}
\expandafter\def\csname faicon@heart\endcsname{{\FAtwo\symbol{151}}}
\expandafter\def\csname faicon@heart-o\endcsname{{\FAtwo\symbol{152}}}
\expandafter\def\csname faicon@home\endcsname{{\FAtwo\symbol{153}}}
\expandafter\def\csname faicon@hospital-o\endcsname{{\FAtwo\symbol{154}}}
\expandafter\def\csname faicon@html5\endcsname{{\FAtwo\symbol{155}}}
\expandafter\def\csname faicon@inbox\endcsname{{\FAtwo\symbol{156}}}
\expandafter\def\csname faicon@outdent\endcsname{{\FAtwo\symbol{157}}}
\expandafter\def\csname faicon@indent\endcsname{{\FAtwo\symbol{158}}}
\expandafter\def\csname faicon@info-circle\endcsname{{\FAtwo\symbol{159}}}
\expandafter\def\csname faicon@inr\endcsname{{\FAtwo\symbol{160}}}
\expandafter\def\csname faicon@instagram\endcsname{{\FAtwo\symbol{161}}}
\expandafter\def\csname faicon@italic\endcsname{{\FAtwo\symbol{162}}}
\expandafter\def\csname faicon@jpy\endcsname{{\FAtwo\symbol{163}}}
\expandafter\def\csname faicon@key\endcsname{{\FAtwo\symbol{164}}}
\expandafter\def\csname faicon@keyboard-o\endcsname{{\FAtwo\symbol{165}}}
\expandafter\def\csname faicon@krw\endcsname{{\FAtwo\symbol{166}}}
\expandafter\def\csname faicon@laptop\endcsname{{\FAtwo\symbol{167}}}
\expandafter\def\csname faicon@leaf\endcsname{{\FAtwo\symbol{168}}}
\expandafter\def\csname faicon@gavel\endcsname{{\FAtwo\symbol{169}}}
\expandafter\def\csname faicon@lemon-o\endcsname{{\FAtwo\symbol{170}}}
\expandafter\def\csname faicon@level-down\endcsname{{\FAtwo\symbol{171}}}
\expandafter\def\csname faicon@level-up\endcsname{{\FAtwo\symbol{172}}}
\expandafter\def\csname faicon@lightbulb-o\endcsname{{\FAtwo\symbol{173}}}
\expandafter\def\csname faicon@link\endcsname{{\FAtwo\symbol{174}}}
\expandafter\def\csname faicon@linkedin\endcsname{{\FAtwo\symbol{175}}}
\expandafter\def\csname faicon@linkedin-square\endcsname{{\FAtwo\symbol{176}}}
\expandafter\def\csname faicon@linux\endcsname{{\FAtwo\symbol{177}}}
\expandafter\def\csname faicon@list\endcsname{{\FAtwo\symbol{178}}}
\expandafter\def\csname faicon@list-alt\endcsname{{\FAtwo\symbol{179}}}
\expandafter\def\csname faicon@location-arrow\endcsname{{\FAtwo\symbol{180}}}
\expandafter\def\csname faicon@lock\endcsname{{\FAtwo\symbol{181}}}
\expandafter\def\csname faicon@long-arrow-down\endcsname{{\FAtwo\symbol{182}}}
\expandafter\def\csname faicon@long-arrow-left\endcsname{{\FAtwo\symbol{183}}}
\expandafter\def\csname faicon@long-arrow-right\endcsname{{\FAtwo\symbol{184}}}
\expandafter\def\csname faicon@long-arrow-up\endcsname{{\FAtwo\symbol{185}}}
\expandafter\def\csname faicon@magic\endcsname{{\FAtwo\symbol{186}}}
\expandafter\def\csname faicon@magnet\endcsname{{\FAtwo\symbol{187}}}
\expandafter\def\csname faicon@male\endcsname{{\FAtwo\symbol{188}}}
\expandafter\def\csname faicon@map-marker\endcsname{{\FAtwo\symbol{189}}}
\expandafter\def\csname faicon@maxcdn\endcsname{{\FAtwo\symbol{190}}}
\expandafter\def\csname faicon@medkit\endcsname{{\FAtwo\symbol{191}}}
\expandafter\def\csname faicon@meh-o\endcsname{{\FAtwo\symbol{192}}}
\expandafter\def\csname faicon@microphone\endcsname{{\FAtwo\symbol{193}}}
\expandafter\def\csname faicon@microphone-slash\endcsname{{\FAtwo\symbol{194}}}
\expandafter\def\csname faicon@minus\endcsname{{\FAtwo\symbol{195}}}
\expandafter\def\csname faicon@minus-circle\endcsname{{\FAtwo\symbol{196}}}
\expandafter\def\csname faicon@minus-square\endcsname{{\FAtwo\symbol{197}}}
\expandafter\def\csname faicon@mobile\endcsname{{\FAtwo\symbol{198}}}
\expandafter\def\csname faicon@money\endcsname{{\FAtwo\symbol{199}}}
\expandafter\def\csname faicon@arrows\endcsname{{\FAtwo\symbol{200}}}
\expandafter\def\csname faicon@music\endcsname{{\FAtwo\symbol{201}}}
\expandafter\def\csname faicon@power-off\endcsname{{\FAtwo\symbol{202}}}
\expandafter\def\csname faicon@check\endcsname{{\FAtwo\symbol{203}}}
\expandafter\def\csname faicon@check-circle-o\endcsname{{\FAtwo\symbol{204}}}
\expandafter\def\csname faicon@check-circle\endcsname{{\FAtwo\symbol{205}}}
\expandafter\def\csname faicon@list-ol\endcsname{{\FAtwo\symbol{206}}}
\expandafter\def\csname faicon@paperclip\endcsname{{\FAtwo\symbol{207}}}
\expandafter\def\csname faicon@clipboard\endcsname{{\FAtwo\symbol{208}}}
\expandafter\def\csname faicon@pause\endcsname{{\FAtwo\symbol{209}}}
\expandafter\def\csname faicon@pencil\endcsname{{\FAtwo\symbol{210}}}
\expandafter\def\csname faicon@phone\endcsname{{\FAtwo\symbol{211}}}
\expandafter\def\csname faicon@phone-square\endcsname{{\FAtwo\symbol{212}}}
\expandafter\def\csname faicon@picture-o\endcsname{{\FAtwo\symbol{213}}}
\expandafter\def\csname faicon@pinterest\endcsname{{\FAtwo\symbol{214}}}
\expandafter\def\csname faicon@pinterest-square\endcsname{{\FAtwo\symbol{215}}}
\expandafter\def\csname faicon@plane\endcsname{{\FAtwo\symbol{216}}}
\expandafter\def\csname faicon@play\endcsname{{\FAtwo\symbol{217}}}
\expandafter\def\csname faicon@play-circle-o\endcsname{{\FAtwo\symbol{218}}}
\expandafter\def\csname faicon@play-circle\endcsname{{\FAtwo\symbol{219}}}
\expandafter\def\csname faicon@plus\endcsname{{\FAtwo\symbol{220}}}
\expandafter\def\csname faicon@plus-circle\endcsname{{\FAtwo\symbol{221}}}
\expandafter\def\csname faicon@plus-square-o\endcsname{{\FAtwo\symbol{222}}}
\expandafter\def\csname faicon@print\endcsname{{\FAtwo\symbol{223}}}
\expandafter\def\csname faicon@thumb-tack\endcsname{{\FAtwo\symbol{224}}}
\expandafter\def\csname faicon@puzzle-piece\endcsname{{\FAtwo\symbol{225}}}
\expandafter\def\csname faicon@qrcode\endcsname{{\FAtwo\symbol{226}}}
\expandafter\def\csname faicon@question\endcsname{{\FAtwo\symbol{227}}}
\expandafter\def\csname faicon@question-circle\endcsname{{\FAtwo\symbol{228}}}
\expandafter\def\csname faicon@quote-left\endcsname{{\FAtwo\symbol{229}}}
\expandafter\def\csname faicon@quote-right\endcsname{{\FAtwo\symbol{230}}}
\expandafter\def\csname faicon@random\endcsname{{\FAtwo\symbol{231}}}
\expandafter\def\csname faicon@refresh\endcsname{{\FAtwo\symbol{232}}}
\expandafter\def\csname faicon@times\endcsname{{\FAtwo\symbol{233}}}
\expandafter\def\csname faicon@times-circle-o\endcsname{{\FAtwo\symbol{234}}}
\expandafter\def\csname faicon@times-circle\endcsname{{\FAtwo\symbol{235}}}
\expandafter\def\csname faicon@renren\endcsname{{\FAtwo\symbol{236}}}
\expandafter\def\csname faicon@bars\endcsname{{\FAtwo\symbol{237}}}
\expandafter\def\csname faicon@repeat\endcsname{{\FAtwo\symbol{238}}}
\expandafter\def\csname faicon@reply\endcsname{{\FAtwo\symbol{239}}}
\expandafter\def\csname faicon@reply-all\endcsname{{\FAtwo\symbol{240}}}
\expandafter\def\csname faicon@expand\endcsname{{\FAtwo\symbol{241}}}
\expandafter\def\csname faicon@arrows-h\endcsname{{\FAtwo\symbol{242}}}
\expandafter\def\csname faicon@compress\endcsname{{\FAtwo\symbol{243}}}
\expandafter\def\csname faicon@arrows-v\endcsname{{\FAtwo\symbol{244}}}
\expandafter\def\csname faicon@retweet\endcsname{{\FAtwo\symbol{245}}}
\expandafter\def\csname faicon@road\endcsname{{\FAtwo\symbol{246}}}
\expandafter\def\csname faicon@rocket\endcsname{{\FAtwo\symbol{247}}}
\expandafter\def\csname faicon@rss\endcsname{{\FAtwo\symbol{248}}}
\expandafter\def\csname faicon@rub\endcsname{{\FAtwo\symbol{249}}}
\expandafter\def\csname faicon@floppy-o\endcsname{{\FAtwo\symbol{250}}}
\expandafter\def\csname faicon@crosshairs\endcsname{{\FAtwo\symbol{251}}}
\expandafter\def\csname faicon@search\endcsname{{\FAtwo\symbol{252}}}
\expandafter\def\csname faicon@share-square-o\endcsname{{\FAtwo\symbol{253}}}
\expandafter\def\csname faicon@share\endcsname{{\FAtwo\symbol{254}}}
\expandafter\def\csname faicon@share-square\endcsname{{\FAtwo\symbol{255}}}
\expandafter\def\csname faicon@shield\endcsname{{\FAthree\symbol{0}}}
\expandafter\def\csname faicon@shopping-cart\endcsname{{\FAthree\symbol{1}}}
\expandafter\def\csname faicon@square\endcsname{{\FAthree\symbol{2}}}
\expandafter\def\csname faicon@signal\endcsname{{\FAthree\symbol{3}}}
\expandafter\def\csname faicon@sign-in\endcsname{{\FAthree\symbol{4}}}
\expandafter\def\csname faicon@sign-out\endcsname{{\FAthree\symbol{5}}}
\expandafter\def\csname faicon@sitemap\endcsname{{\FAthree\symbol{6}}}
\expandafter\def\csname faicon@skype\endcsname{{\FAthree\symbol{7}}}
\expandafter\def\csname faicon@smile-o\endcsname{{\FAthree\symbol{8}}}
\expandafter\def\csname faicon@sort\endcsname{{\FAthree\symbol{9}}}
\expandafter\def\csname faicon@sort-alpha-asc\endcsname{{\FAthree\symbol{10}}}
\expandafter\def\csname faicon@sort-amount-asc\endcsname{{\FAthree\symbol{11}}}
\expandafter\def\csname faicon@sort-amount-desc\endcsname{{\FAthree\symbol{12}}}
\expandafter\def\csname faicon@sort-numeric-asc\endcsname{{\FAthree\symbol{13}}}
\expandafter\def\csname faicon@sort-numeric-desc\endcsname{{\FAthree\symbol{14}}}
\expandafter\def\csname faicon@sort-desc\endcsname{{\FAthree\symbol{15}}}
\expandafter\def\csname faicon@sort-asc\endcsname{{\FAthree\symbol{16}}}
\expandafter\def\csname faicon@spinner\endcsname{{\FAthree\symbol{17}}}
\expandafter\def\csname faicon@stack-exchange\endcsname{{\FAthree\symbol{18}}}
\expandafter\def\csname faicon@stack-overflow\endcsname{{\FAthree\symbol{19}}}
\expandafter\def\csname faicon@star\endcsname{{\FAthree\symbol{20}}}
\expandafter\def\csname faicon@star-o\endcsname{{\FAthree\symbol{21}}}
\expandafter\def\csname faicon@star-half\endcsname{{\FAthree\symbol{22}}}
\expandafter\def\csname faicon@star-half-o\endcsname{{\FAthree\symbol{23}}}
\expandafter\def\csname faicon@step-backward\endcsname{{\FAthree\symbol{24}}}
\expandafter\def\csname faicon@step-forward\endcsname{{\FAthree\symbol{25}}}
\expandafter\def\csname faicon@stethoscope\endcsname{{\FAthree\symbol{26}}}
\expandafter\def\csname faicon@stop\endcsname{{\FAthree\symbol{27}}}
\expandafter\def\csname faicon@strikethrough\endcsname{{\FAthree\symbol{28}}}
\expandafter\def\csname faicon@subscript\endcsname{{\FAthree\symbol{29}}}
\expandafter\def\csname faicon@suitcase\endcsname{{\FAthree\symbol{30}}}
\expandafter\def\csname faicon@sun-o\endcsname{{\FAthree\symbol{31}}}
\expandafter\def\csname faicon@superscript\endcsname{{\FAthree\symbol{32}}}
\expandafter\def\csname faicon@table\endcsname{{\FAthree\symbol{33}}}
\expandafter\def\csname faicon@tablet\endcsname{{\FAthree\symbol{34}}}
\expandafter\def\csname faicon@tag\endcsname{{\FAthree\symbol{35}}}
\expandafter\def\csname faicon@tags\endcsname{{\FAthree\symbol{36}}}
\expandafter\def\csname faicon@tasks\endcsname{{\FAthree\symbol{37}}}
\expandafter\def\csname faicon@terminal\endcsname{{\FAthree\symbol{38}}}
\expandafter\def\csname faicon@text-height\endcsname{{\FAthree\symbol{39}}}
\expandafter\def\csname faicon@text-width\endcsname{{\FAthree\symbol{40}}}
\expandafter\def\csname faicon@th\endcsname{{\FAthree\symbol{41}}}
\expandafter\def\csname faicon@th-large\endcsname{{\FAthree\symbol{42}}}
\expandafter\def\csname faicon@th-list\endcsname{{\FAthree\symbol{43}}}
\expandafter\def\csname faicon@thumbs-o-down\endcsname{{\FAthree\symbol{44}}}
\expandafter\def\csname faicon@thumbs-o-up\endcsname{{\FAthree\symbol{45}}}
\expandafter\def\csname faicon@ticket\endcsname{{\FAthree\symbol{46}}}
\expandafter\def\csname faicon@clock-o\endcsname{{\FAthree\symbol{47}}}
\expandafter\def\csname faicon@tint\endcsname{{\FAthree\symbol{48}}}
\expandafter\def\csname faicon@trash-o\endcsname{{\FAthree\symbol{49}}}
\expandafter\def\csname faicon@trello\endcsname{{\FAthree\symbol{50}}}
\expandafter\def\csname faicon@trophy\endcsname{{\FAthree\symbol{51}}}
\expandafter\def\csname faicon@truck\endcsname{{\FAthree\symbol{52}}}
\expandafter\def\csname faicon@tumblr\endcsname{{\FAthree\symbol{53}}}
\expandafter\def\csname faicon@tumblr-square\endcsname{{\FAthree\symbol{54}}}
\expandafter\def\csname faicon@twitter\endcsname{{\FAthree\symbol{55}}}
\expandafter\def\csname faicon@twitter-square\endcsname{{\FAthree\symbol{56}}}
\expandafter\def\csname faicon@list-ul\endcsname{{\FAthree\symbol{57}}}
\expandafter\def\csname faicon@umbrella\endcsname{{\FAthree\symbol{58}}}
\expandafter\def\csname faicon@underline\endcsname{{\FAthree\symbol{59}}}
\expandafter\def\csname faicon@undo\endcsname{{\FAthree\symbol{60}}}
\expandafter\def\csname faicon@google\endcsname{{\FAthree\symbol{61}}}
\expandafter\def\csname faicon@paw\endcsname{{\FAthree\symbol{62}}}
\expandafter\def\csname faicon@database\endcsname{{\FAthree\symbol{63}}}
\expandafter\def\csname faicon@file-pdf-o\endcsname{{\FAthree\symbol{64}}}
\expandafter\def\csname faicon@rebel\endcsname{{\FAthree\symbol{65}}}
\expandafter\def\csname faicon@empire\endcsname{{\FAthree\symbol{66}}}
\expandafter\def\csname faicon@git-square\endcsname{{\FAthree\symbol{67}}}
\expandafter\def\csname faicon@tencent-weibo\endcsname{{\FAthree\symbol{68}}}
\expandafter\def\csname faicon@qq\endcsname{{\FAthree\symbol{69}}}
\expandafter\def\csname faicon@weixin\endcsname{{\FAthree\symbol{70}}}
\expandafter\def\csname faicon@share-alt\endcsname{{\FAthree\symbol{71}}}
\expandafter\def\csname faicon@cc-visa\endcsname{{\FAthree\symbol{72}}}
\expandafter\def\csname faicon@fonticons\endcsname{{\FAthree\symbol{73}}}
\expandafter\def\csname faicon@reddit-alien\endcsname{{\FAthree\symbol{74}}}
\expandafter\def\csname faicon@modx\endcsname{{\FAthree\symbol{75}}}
\expandafter\def\csname faicon@fort-awesome\endcsname{{\FAthree\symbol{76}}}
\expandafter\def\csname faicon@volume-control-phone\endcsname{{\FAthree\symbol{77}}}
\expandafter\def\csname faicon@braille\endcsname{{\FAthree\symbol{78}}}
\expandafter\def\csname faicon@assistive-listening-systems\endcsname{{\FAthree\symbol{79}}}
\expandafter\def\csname faicon@american-sign-language-interpreting\endcsname{{\FAthree\symbol{80}}}
\expandafter\def\csname faicon@deaf\endcsname{{\FAthree\symbol{81}}}
\expandafter\def\csname faicon@glide\endcsname{{\FAthree\symbol{82}}}
\expandafter\def\csname faicon@glide-g\endcsname{{\FAthree\symbol{83}}}
\expandafter\def\csname faicon@sign-language\endcsname{{\FAthree\symbol{84}}}
\expandafter\def\csname faicon@low-vision\endcsname{{\FAthree\symbol{85}}}
\expandafter\def\csname faicon@viadeo\endcsname{{\FAthree\symbol{86}}}
\expandafter\def\csname faicon@viadeo-square\endcsname{{\FAthree\symbol{87}}}
\expandafter\def\csname faicon@snapchat\endcsname{{\FAthree\symbol{88}}}
\expandafter\def\csname faicon@snapchat-ghost\endcsname{{\FAthree\symbol{89}}}
\expandafter\def\csname faicon@snapchat-square\endcsname{{\FAthree\symbol{90}}}
\expandafter\def\csname faicon@pied-piper\endcsname{{\FAthree\symbol{91}}}
\expandafter\def\csname faicon@first-order\endcsname{{\FAthree\symbol{92}}}
\expandafter\def\csname faicon@yoast\endcsname{{\FAthree\symbol{93}}}
\expandafter\def\csname faicon@themeisle\endcsname{{\FAthree\symbol{94}}}
\expandafter\def\csname faicon@google-plus-official\endcsname{{\FAthree\symbol{95}}}
\expandafter\def\csname faicon@font-awesome\endcsname{{\FAthree\symbol{96}}}
\expandafter\def\csname faicon@chain-broken\endcsname{{\FAthree\symbol{97}}}
\expandafter\def\csname faicon@unlock\endcsname{{\FAthree\symbol{98}}}
\expandafter\def\csname faicon@unlock-alt\endcsname{{\FAthree\symbol{99}}}
\expandafter\def\csname faicon@arrow-circle-o-up\endcsname{{\FAthree\symbol{100}}}
\expandafter\def\csname faicon@upload\endcsname{{\FAthree\symbol{101}}}
\expandafter\def\csname faicon@usd\endcsname{{\FAthree\symbol{102}}}
\expandafter\def\csname faicon@user\endcsname{{\FAthree\symbol{103}}}
\expandafter\def\csname faicon@user-md\endcsname{{\FAthree\symbol{104}}}
\expandafter\def\csname faicon@venus\endcsname{{\FAthree\symbol{105}}}
\expandafter\def\csname faicon@vimeo-square\endcsname{{\FAthree\symbol{106}}}
\expandafter\def\csname faicon@vk\endcsname{{\FAthree\symbol{107}}}
\expandafter\def\csname faicon@volume-down\endcsname{{\FAthree\symbol{108}}}
\expandafter\def\csname faicon@volume-off\endcsname{{\FAthree\symbol{109}}}
\expandafter\def\csname faicon@volume-up\endcsname{{\FAthree\symbol{110}}}
\expandafter\def\csname faicon@exclamation-triangle\endcsname{{\FAthree\symbol{111}}}
\expandafter\def\csname faicon@weibo\endcsname{{\FAthree\symbol{112}}}
\expandafter\def\csname faicon@windows\endcsname{{\FAthree\symbol{113}}}
\expandafter\def\csname faicon@wrench\endcsname{{\FAthree\symbol{114}}}
\expandafter\def\csname faicon@xing\endcsname{{\FAthree\symbol{115}}}
\expandafter\def\csname faicon@xing-square\endcsname{{\FAthree\symbol{116}}}
\expandafter\def\csname faicon@youtube\endcsname{{\FAthree\symbol{117}}}
\expandafter\def\csname faicon@youtube-play\endcsname{{\FAthree\symbol{118}}}
\expandafter\def\csname faicon@youtube-square\endcsname{{\FAthree\symbol{119}}}
\expandafter\def\csname faicon@search-plus\endcsname{{\FAthree\symbol{120}}}
\expandafter\def\csname faicon@search-minus\endcsname{{\FAthree\symbol{121}}}

%% end of file `fontawesomesymbols-pdftex.tex'.


==> fontawesomesymbols-xeluatex.tex <==
\expandafter\def\csname faicon@glass\endcsname{{\FA\symbol{"F000}}}
\expandafter\def\csname faicon@music\endcsname{{\FA\symbol{"F001}}}
\expandafter\def\csname faicon@search\endcsname{{\FA\symbol{"F002}}}
\expandafter\def\csname faicon@envelope-o\endcsname{{\FA\symbol{"F003}}}
\expandafter\def\csname faicon@heart\endcsname{{\FA\symbol{"F004}}}
\expandafter\def\csname faicon@star\endcsname{{\FA\symbol{"F005}}}
\expandafter\def\csname faicon@star-o\endcsname{{\FA\symbol{"F006}}}
\expandafter\def\csname faicon@user\endcsname{{\FA\symbol{"F007}}}
\expandafter\def\csname faicon@film\endcsname{{\FA\symbol{"F008}}}
\expandafter\def\csname faicon@th-large\endcsname{{\FA\symbol{"F009}}}
\expandafter\def\csname faicon@th\endcsname{{\FA\symbol{"F00A}}}
\expandafter\def\csname faicon@th-list\endcsname{{\FA\symbol{"F00B}}}
\expandafter\def\csname faicon@check\endcsname{{\FA\symbol{"F00C}}}
\expandafter\def\csname faicon@times\endcsname{{\FA\symbol{"F00D}}}
\expandafter\def\csname faicon@search-plus\endcsname{{\FA\symbol{"F00E}}}
\expandafter\def\csname faicon@search-minus\endcsname{{\FA\symbol{"F010}}}
\expandafter\def\csname faicon@power-off\endcsname{{\FA\symbol{"F011}}}
\expandafter\def\csname faicon@signal\endcsname{{\FA\symbol{"F012}}}
\expandafter\def\csname faicon@cog\endcsname{{\FA\symbol{"F013}}}
\expandafter\def\csname faicon@trash-o\endcsname{{\FA\symbol{"F014}}}
\expandafter\def\csname faicon@home\endcsname{{\FA\symbol{"F015}}}
\expandafter\def\csname faicon@file-o\endcsname{{\FA\symbol{"F016}}}
\expandafter\def\csname faicon@clock-o\endcsname{{\FA\symbol{"F017}}}
\expandafter\def\csname faicon@road\endcsname{{\FA\symbol{"F018}}}
\expandafter\def\csname faicon@download\endcsname{{\FA\symbol{"F019}}}
\expandafter\def\csname faicon@arrow-circle-o-down\endcsname{{\FA\symbol{"F01A}}}
\expandafter\def\csname faicon@arrow-circle-o-up\endcsname{{\FA\symbol{"F01B}}}
\expandafter\def\csname faicon@inbox\endcsname{{\FA\symbol{"F01C}}}
\expandafter\def\csname faicon@play-circle-o\endcsname{{\FA\symbol{"F01D}}}
\expandafter\def\csname faicon@repeat\endcsname{{\FA\symbol{"F01E}}}
\expandafter\def\csname faicon@refresh\endcsname{{\FA\symbol{"F021}}}
\expandafter\def\csname faicon@list-alt\endcsname{{\FA\symbol{"F022}}}
\expandafter\def\csname faicon@lock\endcsname{{\FA\symbol{"F023}}}
\expandafter\def\csname faicon@flag\endcsname{{\FA\symbol{"F024}}}
\expandafter\def\csname faicon@headphones\endcsname{{\FA\symbol{"F025}}}
\expandafter\def\csname faicon@volume-off\endcsname{{\FA\symbol{"F026}}}
\expandafter\def\csname faicon@volume-down\endcsname{{\FA\symbol{"F027}}}
\expandafter\def\csname faicon@volume-up\endcsname{{\FA\symbol{"F028}}}
\expandafter\def\csname faicon@qrcode\endcsname{{\FA\symbol{"F029}}}
\expandafter\def\csname faicon@barcode\endcsname{{\FA\symbol{"F02A}}}
\expandafter\def\csname faicon@tag\endcsname{{\FA\symbol{"F02B}}}
\expandafter\def\csname faicon@tags\endcsname{{\FA\symbol{"F02C}}}
\expandafter\def\csname faicon@book\endcsname{{\FA\symbol{"F02D}}}
\expandafter\def\csname faicon@bookmark\endcsname{{\FA\symbol{"F02E}}}
\expandafter\def\csname faicon@print\endcsname{{\FA\symbol{"F02F}}}
\expandafter\def\csname faicon@camera\endcsname{{\FA\symbol{"F030}}}
\expandafter\def\csname faicon@font\endcsname{{\FA\symbol{"F031}}}
\expandafter\def\csname faicon@bold\endcsname{{\FA\symbol{"F032}}}
\expandafter\def\csname faicon@italic\endcsname{{\FA\symbol{"F033}}}
\expandafter\def\csname faicon@text-height\endcsname{{\FA\symbol{"F034}}}
\expandafter\def\csname faicon@text-width\endcsname{{\FA\symbol{"F035}}}
\expandafter\def\csname faicon@align-left\endcsname{{\FA\symbol{"F036}}}
\expandafter\def\csname faicon@align-center\endcsname{{\FA\symbol{"F037}}}
\expandafter\def\csname faicon@align-right\endcsname{{\FA\symbol{"F038}}}
\expandafter\def\csname faicon@align-justify\endcsname{{\FA\symbol{"F039}}}
\expandafter\def\csname faicon@list\endcsname{{\FA\symbol{"F03A}}}
\expandafter\def\csname faicon@outdent\endcsname{{\FA\symbol{"F03B}}}
\expandafter\def\csname faicon@indent\endcsname{{\FA\symbol{"F03C}}}
\expandafter\def\csname faicon@video-camera\endcsname{{\FA\symbol{"F03D}}}
\expandafter\def\csname faicon@picture-o\endcsname{{\FA\symbol{"F03E}}}
\expandafter\def\csname faicon@pencil\endcsname{{\FA\symbol{"F040}}}
\expandafter\def\csname faicon@map-marker\endcsname{{\FA\symbol{"F041}}}
\expandafter\def\csname faicon@adjust\endcsname{{\FA\symbol{"F042}}}
\expandafter\def\csname faicon@tint\endcsname{{\FA\symbol{"F043}}}
\expandafter\def\csname faicon@pencil-square-o\endcsname{{\FA\symbol{"F044}}}
\expandafter\def\csname faicon@share-square-o\endcsname{{\FA\symbol{"F045}}}
\expandafter\def\csname faicon@check-square-o\endcsname{{\FA\symbol{"F046}}}
\expandafter\def\csname faicon@arrows\endcsname{{\FA\symbol{"F047}}}
\expandafter\def\csname faicon@step-backward\endcsname{{\FA\symbol{"F048}}}
\expandafter\def\csname faicon@fast-backward\endcsname{{\FA\symbol{"F049}}}
\expandafter\def\csname faicon@backward\endcsname{{\FA\symbol{"F04A}}}
\expandafter\def\csname faicon@play\endcsname{{\FA\symbol{"F04B}}}
\expandafter\def\csname faicon@pause\endcsname{{\FA\symbol{"F04C}}}
\expandafter\def\csname faicon@stop\endcsname{{\FA\symbol{"F04D}}}
\expandafter\def\csname faicon@forward\endcsname{{\FA\symbol{"F04E}}}
\expandafter\def\csname faicon@fast-forward\endcsname{{\FA\symbol{"F050}}}
\expandafter\def\csname faicon@step-forward\endcsname{{\FA\symbol{"F051}}}
\expandafter\def\csname faicon@eject\endcsname{{\FA\symbol{"F052}}}
\expandafter\def\csname faicon@chevron-left\endcsname{{\FA\symbol{"F053}}}
\expandafter\def\csname faicon@chevron-right\endcsname{{\FA\symbol{"F054}}}
\expandafter\def\csname faicon@plus-circle\endcsname{{\FA\symbol{"F055}}}
\expandafter\def\csname faicon@minus-circle\endcsname{{\FA\symbol{"F056}}}
\expandafter\def\csname faicon@times-circle\endcsname{{\FA\symbol{"F057}}}
\expandafter\def\csname faicon@check-circle\endcsname{{\FA\symbol{"F058}}}
\expandafter\def\csname faicon@question-circle\endcsname{{\FA\symbol{"F059}}}
\expandafter\def\csname faicon@info-circle\endcsname{{\FA\symbol{"F05A}}}
\expandafter\def\csname faicon@crosshairs\endcsname{{\FA\symbol{"F05B}}}
\expandafter\def\csname faicon@times-circle-o\endcsname{{\FA\symbol{"F05C}}}
\expandafter\def\csname faicon@check-circle-o\endcsname{{\FA\symbol{"F05D}}}
\expandafter\def\csname faicon@ban\endcsname{{\FA\symbol{"F05E}}}
\expandafter\def\csname faicon@arrow-left\endcsname{{\FA\symbol{"F060}}}
\expandafter\def\csname faicon@arrow-right\endcsname{{\FA\symbol{"F061}}}
\expandafter\def\csname faicon@arrow-up\endcsname{{\FA\symbol{"F062}}}
\expandafter\def\csname faicon@arrow-down\endcsname{{\FA\symbol{"F063}}}
\expandafter\def\csname faicon@share\endcsname{{\FA\symbol{"F064}}}
\expandafter\def\csname faicon@expand\endcsname{{\FA\symbol{"F065}}}
\expandafter\def\csname faicon@compress\endcsname{{\FA\symbol{"F066}}}
\expandafter\def\csname faicon@plus\endcsname{{\FA\symbol{"F067}}}
\expandafter\def\csname faicon@minus\endcsname{{\FA\symbol{"F068}}}
\expandafter\def\csname faicon@asterisk\endcsname{{\FA\symbol{"F069}}}
\expandafter\def\csname faicon@exclamation-circle\endcsname{{\FA\symbol{"F06A}}}
\expandafter\def\csname faicon@gift\endcsname{{\FA\symbol{"F06B}}}
\expandafter\def\csname faicon@leaf\endcsname{{\FA\symbol{"F06C}}}
\expandafter\def\csname faicon@fire\endcsname{{\FA\symbol{"F06D}}}
\expandafter\def\csname faicon@eye\endcsname{{\FA\symbol{"F06E}}}
\expandafter\def\csname faicon@eye-slash\endcsname{{\FA\symbol{"F070}}}
\expandafter\def\csname faicon@exclamation-triangle\endcsname{{\FA\symbol{"F071}}}
\expandafter\def\csname faicon@plane\endcsname{{\FA\symbol{"F072}}}
\expandafter\def\csname faicon@calendar\endcsname{{\FA\symbol{"F073}}}
\expandafter\def\csname faicon@random\endcsname{{\FA\symbol{"F074}}}
\expandafter\def\csname faicon@comment\endcsname{{\FA\symbol{"F075}}}
\expandafter\def\csname faicon@magnet\endcsname{{\FA\symbol{"F076}}}
\expandafter\def\csname faicon@chevron-up\endcsname{{\FA\symbol{"F077}}}
\expandafter\def\csname faicon@chevron-down\endcsname{{\FA\symbol{"F078}}}
\expandafter\def\csname faicon@retweet\endcsname{{\FA\symbol{"F079}}}
\expandafter\def\csname faicon@shopping-cart\endcsname{{\FA\symbol{"F07A}}}
\expandafter\def\csname faicon@folder\endcsname{{\FA\symbol{"F07B}}}
\expandafter\def\csname faicon@folder-open\endcsname{{\FA\symbol{"F07C}}}
\expandafter\def\csname faicon@arrows-v\endcsname{{\FA\symbol{"F07D}}}
\expandafter\def\csname faicon@arrows-h\endcsname{{\FA\symbol{"F07E}}}
\expandafter\def\csname faicon@bar-chart\endcsname{{\FA\symbol{"F080}}}
\expandafter\def\csname faicon@twitter-square\endcsname{{\FA\symbol{"F081}}}
\expandafter\def\csname faicon@facebook-square\endcsname{{\FA\symbol{"F082}}}
\expandafter\def\csname faicon@camera-retro\endcsname{{\FA\symbol{"F083}}}
\expandafter\def\csname faicon@key\endcsname{{\FA\symbol{"F084}}}
\expandafter\def\csname faicon@cogs\endcsname{{\FA\symbol{"F085}}}
\expandafter\def\csname faicon@comments\endcsname{{\FA\symbol{"F086}}}
\expandafter\def\csname faicon@thumbs-o-up\endcsname{{\FA\symbol{"F087}}}
\expandafter\def\csname faicon@thumbs-o-down\endcsname{{\FA\symbol{"F088}}}
\expandafter\def\csname faicon@star-half\endcsname{{\FA\symbol{"F089}}}
\expandafter\def\csname faicon@heart-o\endcsname{{\FA\symbol{"F08A}}}
\expandafter\def\csname faicon@sign-out\endcsname{{\FA\symbol{"F08B}}}
\expandafter\def\csname faicon@linkedin-square\endcsname{{\FA\symbol{"F08C}}}
\expandafter\def\csname faicon@thumb-tack\endcsname{{\FA\symbol{"F08D}}}
\expandafter\def\csname faicon@external-link\endcsname{{\FA\symbol{"F08E}}}
\expandafter\def\csname faicon@sign-in\endcsname{{\FA\symbol{"F090}}}
\expandafter\def\csname faicon@trophy\endcsname{{\FA\symbol{"F091}}}
\expandafter\def\csname faicon@github-square\endcsname{{\FA\symbol{"F092}}}
\expandafter\def\csname faicon@upload\endcsname{{\FA\symbol{"F093}}}
\expandafter\def\csname faicon@lemon-o\endcsname{{\FA\symbol{"F094}}}
\expandafter\def\csname faicon@phone\endcsname{{\FA\symbol{"F095}}}
\expandafter\def\csname faicon@square-o\endcsname{{\FA\symbol{"F096}}}
\expandafter\def\csname faicon@bookmark-o\endcsname{{\FA\symbol{"F097}}}
\expandafter\def\csname faicon@phone-square\endcsname{{\FA\symbol{"F098}}}
\expandafter\def\csname faicon@twitter\endcsname{{\FA\symbol{"F099}}}
\expandafter\def\csname faicon@facebook\endcsname{{\FA\symbol{"F09A}}}
\expandafter\def\csname faicon@github\endcsname{{\FA\symbol{"F09B}}}
\expandafter\def\csname faicon@unlock\endcsname{{\FA\symbol{"F09C}}}
\expandafter\def\csname faicon@credit-card\endcsname{{\FA\symbol{"F09D}}}
\expandafter\def\csname faicon@rss\endcsname{{\FA\symbol{"F09E}}}
\expandafter\def\csname faicon@hdd-o\endcsname{{\FA\symbol{"F0A0}}}
\expandafter\def\csname faicon@bullhorn\endcsname{{\FA\symbol{"F0A1}}}
\expandafter\def\csname faicon@bell\endcsname{{\FA\symbol{"F0F3}}}
\expandafter\def\csname faicon@certificate\endcsname{{\FA\symbol{"F0A3}}}
\expandafter\def\csname faicon@hand-o-right\endcsname{{\FA\symbol{"F0A4}}}
\expandafter\def\csname faicon@hand-o-left\endcsname{{\FA\symbol{"F0A5}}}
\expandafter\def\csname faicon@hand-o-up\endcsname{{\FA\symbol{"F0A6}}}
\expandafter\def\csname faicon@hand-o-down\endcsname{{\FA\symbol{"F0A7}}}
\expandafter\def\csname faicon@arrow-circle-left\endcsname{{\FA\symbol{"F0A8}}}
\expandafter\def\csname faicon@arrow-circle-right\endcsname{{\FA\symbol{"F0A9}}}
\expandafter\def\csname faicon@arrow-circle-up\endcsname{{\FA\symbol{"F0AA}}}
\expandafter\def\csname faicon@arrow-circle-down\endcsname{{\FA\symbol{"F0AB}}}
\expandafter\def\csname faicon@globe\endcsname{{\FA\symbol{"F0AC}}}
\expandafter\def\csname faicon@wrench\endcsname{{\FA\symbol{"F0AD}}}
\expandafter\def\csname faicon@tasks\endcsname{{\FA\symbol{"F0AE}}}
\expandafter\def\csname faicon@filter\endcsname{{\FA\symbol{"F0B0}}}
\expandafter\def\csname faicon@briefcase\endcsname{{\FA\symbol{"F0B1}}}
\expandafter\def\csname faicon@arrows-alt\endcsname{{\FA\symbol{"F0B2}}}
\expandafter\def\csname faicon@users\endcsname{{\FA\symbol{"F0C0}}}
\expandafter\def\csname faicon@link\endcsname{{\FA\symbol{"F0C1}}}
\expandafter\def\csname faicon@cloud\endcsname{{\FA\symbol{"F0C2}}}
\expandafter\def\csname faicon@flask\endcsname{{\FA\symbol{"F0C3}}}
\expandafter\def\csname faicon@scissors\endcsname{{\FA\symbol{"F0C4}}}
\expandafter\def\csname faicon@files-o\endcsname{{\FA\symbol{"F0C5}}}
\expandafter\def\csname faicon@paperclip\endcsname{{\FA\symbol{"F0C6}}}
\expandafter\def\csname faicon@floppy-o\endcsname{{\FA\symbol{"F0C7}}}
\expandafter\def\csname faicon@square\endcsname{{\FA\symbol{"F0C8}}}
\expandafter\def\csname faicon@bars\endcsname{{\FA\symbol{"F0C9}}}
\expandafter\def\csname faicon@list-ul\endcsname{{\FA\symbol{"F0CA}}}
\expandafter\def\csname faicon@list-ol\endcsname{{\FA\symbol{"F0CB}}}
\expandafter\def\csname faicon@strikethrough\endcsname{{\FA\symbol{"F0CC}}}
\expandafter\def\csname faicon@underline\endcsname{{\FA\symbol{"F0CD}}}
\expandafter\def\csname faicon@table\endcsname{{\FA\symbol{"F0CE}}}
\expandafter\def\csname faicon@magic\endcsname{{\FA\symbol{"F0D0}}}
\expandafter\def\csname faicon@truck\endcsname{{\FA\symbol{"F0D1}}}
\expandafter\def\csname faicon@pinterest\endcsname{{\FA\symbol{"F0D2}}}
\expandafter\def\csname faicon@pinterest-square\endcsname{{\FA\symbol{"F0D3}}}
\expandafter\def\csname faicon@google-plus-square\endcsname{{\FA\symbol{"F0D4}}}
\expandafter\def\csname faicon@google-plus\endcsname{{\FA\symbol{"F0D5}}}
\expandafter\def\csname faicon@money\endcsname{{\FA\symbol{"F0D6}}}
\expandafter\def\csname faicon@caret-down\endcsname{{\FA\symbol{"F0D7}}}
\expandafter\def\csname faicon@caret-up\endcsname{{\FA\symbol{"F0D8}}}
\expandafter\def\csname faicon@caret-left\endcsname{{\FA\symbol{"F0D9}}}
\expandafter\def\csname faicon@caret-right\endcsname{{\FA\symbol{"F0DA}}}
\expandafter\def\csname faicon@columns\endcsname{{\FA\symbol{"F0DB}}}
\expandafter\def\csname faicon@sort\endcsname{{\FA\symbol{"F0DC}}}
\expandafter\def\csname faicon@sort-desc\endcsname{{\FA\symbol{"F0DD}}}
\expandafter\def\csname faicon@sort-asc\endcsname{{\FA\symbol{"F0DE}}}
\expandafter\def\csname faicon@envelope\endcsname{{\FA\symbol{"F0E0}}}
\expandafter\def\csname faicon@linkedin\endcsname{{\FA\symbol{"F0E1}}}
\expandafter\def\csname faicon@undo\endcsname{{\FA\symbol{"F0E2}}}
\expandafter\def\csname faicon@gavel\endcsname{{\FA\symbol{"F0E3}}}
\expandafter\def\csname faicon@tachometer\endcsname{{\FA\symbol{"F0E4}}}
\expandafter\def\csname faicon@comment-o\endcsname{{\FA\symbol{"F0E5}}}
\expandafter\def\csname faicon@comments-o\endcsname{{\FA\symbol{"F0E6}}}
\expandafter\def\csname faicon@bolt\endcsname{{\FA\symbol{"F0E7}}}
\expandafter\def\csname faicon@sitemap\endcsname{{\FA\symbol{"F0E8}}}
\expandafter\def\csname faicon@umbrella\endcsname{{\FA\symbol{"F0E9}}}
\expandafter\def\csname faicon@clipboard\endcsname{{\FA\symbol{"F0EA}}}
\expandafter\def\csname faicon@lightbulb-o\endcsname{{\FA\symbol{"F0EB}}}
\expandafter\def\csname faicon@exchange\endcsname{{\FA\symbol{"F0EC}}}
\expandafter\def\csname faicon@cloud-download\endcsname{{\FA\symbol{"F0ED}}}
\expandafter\def\csname faicon@cloud-upload\endcsname{{\FA\symbol{"F0EE}}}
\expandafter\def\csname faicon@user-md\endcsname{{\FA\symbol{"F0F0}}}
\expandafter\def\csname faicon@stethoscope\endcsname{{\FA\symbol{"F0F1}}}
\expandafter\def\csname faicon@suitcase\endcsname{{\FA\symbol{"F0F2}}}
\expandafter\def\csname faicon@bell-o\endcsname{{\FA\symbol{"F0A2}}}
\expandafter\def\csname faicon@coffee\endcsname{{\FA\symbol{"F0F4}}}
\expandafter\def\csname faicon@cutlery\endcsname{{\FA\symbol{"F0F5}}}
\expandafter\def\csname faicon@file-text-o\endcsname{{\FA\symbol{"F0F6}}}
\expandafter\def\csname faicon@building-o\endcsname{{\FA\symbol{"F0F7}}}
\expandafter\def\csname faicon@hospital-o\endcsname{{\FA\symbol{"F0F8}}}
\expandafter\def\csname faicon@ambulance\endcsname{{\FA\symbol{"F0F9}}}
\expandafter\def\csname faicon@medkit\endcsname{{\FA\symbol{"F0FA}}}
\expandafter\def\csname faicon@fighter-jet\endcsname{{\FA\symbol{"F0FB}}}
\expandafter\def\csname faicon@beer\endcsname{{\FA\symbol{"F0FC}}}
\expandafter\def\csname faicon@h-square\endcsname{{\FA\symbol{"F0FD}}}
\expandafter\def\csname faicon@plus-square\endcsname{{\FA\symbol{"F0FE}}}
\expandafter\def\csname faicon@angle-double-left\endcsname{{\FA\symbol{"F100}}}
\expandafter\def\csname faicon@angle-double-right\endcsname{{\FA\symbol{"F101}}}
\expandafter\def\csname faicon@angle-double-up\endcsname{{\FA\symbol{"F102}}}
\expandafter\def\csname faicon@angle-double-down\endcsname{{\FA\symbol{"F103}}}
\expandafter\def\csname faicon@angle-left\endcsname{{\FA\symbol{"F104}}}
\expandafter\def\csname faicon@angle-right\endcsname{{\FA\symbol{"F105}}}
\expandafter\def\csname faicon@angle-up\endcsname{{\FA\symbol{"F106}}}
\expandafter\def\csname faicon@angle-down\endcsname{{\FA\symbol{"F107}}}
\expandafter\def\csname faicon@desktop\endcsname{{\FA\symbol{"F108}}}
\expandafter\def\csname faicon@laptop\endcsname{{\FA\symbol{"F109}}}
\expandafter\def\csname faicon@tablet\endcsname{{\FA\symbol{"F10A}}}
\expandafter\def\csname faicon@mobile\endcsname{{\FA\symbol{"F10B}}}
\expandafter\def\csname faicon@circle-o\endcsname{{\FA\symbol{"F10C}}}
\expandafter\def\csname faicon@quote-left\endcsname{{\FA\symbol{"F10D}}}
\expandafter\def\csname faicon@quote-right\endcsname{{\FA\symbol{"F10E}}}
\expandafter\def\csname faicon@spinner\endcsname{{\FA\symbol{"F110}}}
\expandafter\def\csname faicon@circle\endcsname{{\FA\symbol{"F111}}}
\expandafter\def\csname faicon@reply\endcsname{{\FA\symbol{"F112}}}
\expandafter\def\csname faicon@github-alt\endcsname{{\FA\symbol{"F113}}}
\expandafter\def\csname faicon@folder-o\endcsname{{\FA\symbol{"F114}}}
\expandafter\def\csname faicon@folder-open-o\endcsname{{\FA\symbol{"F115}}}
\expandafter\def\csname faicon@smile-o\endcsname{{\FA\symbol{"F118}}}
\expandafter\def\csname faicon@frown-o\endcsname{{\FA\symbol{"F119}}}
\expandafter\def\csname faicon@meh-o\endcsname{{\FA\symbol{"F11A}}}
\expandafter\def\csname faicon@gamepad\endcsname{{\FA\symbol{"F11B}}}
\expandafter\def\csname faicon@keyboard-o\endcsname{{\FA\symbol{"F11C}}}
\expandafter\def\csname faicon@flag-o\endcsname{{\FA\symbol{"F11D}}}
\expandafter\def\csname faicon@flag-checkered\endcsname{{\FA\symbol{"F11E}}}
\expandafter\def\csname faicon@terminal\endcsname{{\FA\symbol{"F120}}}
\expandafter\def\csname faicon@code\endcsname{{\FA\symbol{"F121}}}
\expandafter\def\csname faicon@reply-all\endcsname{{\FA\symbol{"F122}}}
\expandafter\def\csname faicon@star-half-o\endcsname{{\FA\symbol{"F123}}}
\expandafter\def\csname faicon@location-arrow\endcsname{{\FA\symbol{"F124}}}
\expandafter\def\csname faicon@crop\endcsname{{\FA\symbol{"F125}}}
\expandafter\def\csname faicon@code-fork\endcsname{{\FA\symbol{"F126}}}
\expandafter\def\csname faicon@chain-broken\endcsname{{\FA\symbol{"F127}}}
\expandafter\def\csname faicon@question\endcsname{{\FA\symbol{"F128}}}
\expandafter\def\csname faicon@info\endcsname{{\FA\symbol{"F129}}}
\expandafter\def\csname faicon@exclamation\endcsname{{\FA\symbol{"F12A}}}
\expandafter\def\csname faicon@superscript\endcsname{{\FA\symbol{"F12B}}}
\expandafter\def\csname faicon@subscript\endcsname{{\FA\symbol{"F12C}}}
\expandafter\def\csname faicon@eraser\endcsname{{\FA\symbol{"F12D}}}
\expandafter\def\csname faicon@puzzle-piece\endcsname{{\FA\symbol{"F12E}}}
\expandafter\def\csname faicon@microphone\endcsname{{\FA\symbol{"F130}}}
\expandafter\def\csname faicon@microphone-slash\endcsname{{\FA\symbol{"F131}}}
\expandafter\def\csname faicon@shield\endcsname{{\FA\symbol{"F132}}}
\expandafter\def\csname faicon@calendar-o\endcsname{{\FA\symbol{"F133}}}
\expandafter\def\csname faicon@fire-extinguisher\endcsname{{\FA\symbol{"F134}}}
\expandafter\def\csname faicon@rocket\endcsname{{\FA\symbol{"F135}}}
\expandafter\def\csname faicon@maxcdn\endcsname{{\FA\symbol{"F136}}}
\expandafter\def\csname faicon@chevron-circle-left\endcsname{{\FA\symbol{"F137}}}
\expandafter\def\csname faicon@chevron-circle-right\endcsname{{\FA\symbol{"F138}}}
\expandafter\def\csname faicon@chevron-circle-up\endcsname{{\FA\symbol{"F139}}}
\expandafter\def\csname faicon@chevron-circle-down\endcsname{{\FA\symbol{"F13A}}}
\expandafter\def\csname faicon@html5\endcsname{{\FA\symbol{"F13B}}}
\expandafter\def\csname faicon@css3\endcsname{{\FA\symbol{"F13C}}}
\expandafter\def\csname faicon@anchor\endcsname{{\FA\symbol{"F13D}}}
\expandafter\def\csname faicon@unlock-alt\endcsname{{\FA\symbol{"F13E}}}
\expandafter\def\csname faicon@bullseye\endcsname{{\FA\symbol{"F140}}}
\expandafter\def\csname faicon@ellipsis-h\endcsname{{\FA\symbol{"F141}}}
\expandafter\def\csname faicon@ellipsis-v\endcsname{{\FA\symbol{"F142}}}
\expandafter\def\csname faicon@rss-square\endcsname{{\FA\symbol{"F143}}}
\expandafter\def\csname faicon@play-circle\endcsname{{\FA\symbol{"F144}}}
\expandafter\def\csname faicon@ticket\endcsname{{\FA\symbol{"F145}}}
\expandafter\def\csname faicon@minus-square\endcsname{{\FA\symbol{"F146}}}
\expandafter\def\csname faicon@minus-square-o\endcsname{{\FA\symbol{"F147}}}
\expandafter\def\csname faicon@level-up\endcsname{{\FA\symbol{"F148}}}
\expandafter\def\csname faicon@level-down\endcsname{{\FA\symbol{"F149}}}
\expandafter\def\csname faicon@check-square\endcsname{{\FA\symbol{"F14A}}}
\expandafter\def\csname faicon@pencil-square\endcsname{{\FA\symbol{"F14B}}}
\expandafter\def\csname faicon@external-link-square\endcsname{{\FA\symbol{"F14C}}}
\expandafter\def\csname faicon@share-square\endcsname{{\FA\symbol{"F14D}}}
\expandafter\def\csname faicon@compass\endcsname{{\FA\symbol{"F14E}}}
\expandafter\def\csname faicon@caret-square-o-down\endcsname{{\FA\symbol{"F150}}}
\expandafter\def\csname faicon@caret-square-o-up\endcsname{{\FA\symbol{"F151}}}
\expandafter\def\csname faicon@caret-square-o-right\endcsname{{\FA\symbol{"F152}}}
\expandafter\def\csname faicon@eur\endcsname{{\FA\symbol{"F153}}}
\expandafter\def\csname faicon@gbp\endcsname{{\FA\symbol{"F154}}}
\expandafter\def\csname faicon@usd\endcsname{{\FA\symbol{"F155}}}
\expandafter\def\csname faicon@inr\endcsname{{\FA\symbol{"F156}}}
\expandafter\def\csname faicon@jpy\endcsname{{\FA\symbol{"F157}}}
\expandafter\def\csname faicon@rub\endcsname{{\FA\symbol{"F158}}}
\expandafter\def\csname faicon@krw\endcsname{{\FA\symbol{"F159}}}
\expandafter\def\csname faicon@btc\endcsname{{\FA\symbol{"F15A}}}
\expandafter\def\csname faicon@file\endcsname{{\FA\symbol{"F15B}}}
\expandafter\def\csname faicon@file-text\endcsname{{\FA\symbol{"F15C}}}
\expandafter\def\csname faicon@sort-alpha-asc\endcsname{{\FA\symbol{"F15D}}}
\expandafter\def\csname faicon@sort-alpha-desc\endcsname{{\FA\symbol{"F15E}}}
\expandafter\def\csname faicon@sort-amount-asc\endcsname{{\FA\symbol{"F160}}}
\expandafter\def\csname faicon@sort-amount-desc\endcsname{{\FA\symbol{"F161}}}
\expandafter\def\csname faicon@sort-numeric-asc\endcsname{{\FA\symbol{"F162}}}
\expandafter\def\csname faicon@sort-numeric-desc\endcsname{{\FA\symbol{"F163}}}
\expandafter\def\csname faicon@thumbs-up\endcsname{{\FA\symbol{"F164}}}
\expandafter\def\csname faicon@thumbs-down\endcsname{{\FA\symbol{"F165}}}
\expandafter\def\csname faicon@youtube-square\endcsname{{\FA\symbol{"F166}}}
\expandafter\def\csname faicon@youtube\endcsname{{\FA\symbol{"F167}}}
\expandafter\def\csname faicon@xing\endcsname{{\FA\symbol{"F168}}}
\expandafter\def\csname faicon@xing-square\endcsname{{\FA\symbol{"F169}}}
\expandafter\def\csname faicon@youtube-play\endcsname{{\FA\symbol{"F16A}}}
\expandafter\def\csname faicon@dropbox\endcsname{{\FA\symbol{"F16B}}}
\expandafter\def\csname faicon@stack-overflow\endcsname{{\FA\symbol{"F16C}}}
\expandafter\def\csname faicon@instagram\endcsname{{\FA\symbol{"F16D}}}
\expandafter\def\csname faicon@flickr\endcsname{{\FA\symbol{"F16E}}}
\expandafter\def\csname faicon@adn\endcsname{{\FA\symbol{"F170}}}
\expandafter\def\csname faicon@bitbucket\endcsname{{\FA\symbol{"F171}}}
\expandafter\def\csname faicon@bitbucket-square\endcsname{{\FA\symbol{"F172}}}
\expandafter\def\csname faicon@tumblr\endcsname{{\FA\symbol{"F173}}}
\expandafter\def\csname faicon@tumblr-square\endcsname{{\FA\symbol{"F174}}}
\expandafter\def\csname faicon@long-arrow-down\endcsname{{\FA\symbol{"F175}}}
\expandafter\def\csname faicon@long-arrow-up\endcsname{{\FA\symbol{"F176}}}
\expandafter\def\csname faicon@long-arrow-left\endcsname{{\FA\symbol{"F177}}}
\expandafter\def\csname faicon@long-arrow-right\endcsname{{\FA\symbol{"F178}}}
\expandafter\def\csname faicon@apple\endcsname{{\FA\symbol{"F179}}}
\expandafter\def\csname faicon@windows\endcsname{{\FA\symbol{"F17A}}}
\expandafter\def\csname faicon@android\endcsname{{\FA\symbol{"F17B}}}
\expandafter\def\csname faicon@linux\endcsname{{\FA\symbol{"F17C}}}
\expandafter\def\csname faicon@dribbble\endcsname{{\FA\symbol{"F17D}}}
\expandafter\def\csname faicon@skype\endcsname{{\FA\symbol{"F17E}}}
\expandafter\def\csname faicon@foursquare\endcsname{{\FA\symbol{"F180}}}
\expandafter\def\csname faicon@trello\endcsname{{\FA\symbol{"F181}}}
\expandafter\def\csname faicon@female\endcsname{{\FA\symbol{"F182}}}
\expandafter\def\csname faicon@male\endcsname{{\FA\symbol{"F183}}}
\expandafter\def\csname faicon@gratipay\endcsname{{\FA\symbol{"F184}}}
\expandafter\def\csname faicon@sun-o\endcsname{{\FA\symbol{"F185}}}
\expandafter\def\csname faicon@moon-o\endcsname{{\FA\symbol{"F186}}}
\expandafter\def\csname faicon@archive\endcsname{{\FA\symbol{"F187}}}
\expandafter\def\csname faicon@bug\endcsname{{\FA\symbol{"F188}}}
\expandafter\def\csname faicon@vk\endcsname{{\FA\symbol{"F189}}}
\expandafter\def\csname faicon@weibo\endcsname{{\FA\symbol{"F18A}}}
\expandafter\def\csname faicon@renren\endcsname{{\FA\symbol{"F18B}}}
\expandafter\def\csname faicon@pagelines\endcsname{{\FA\symbol{"F18C}}}
\expandafter\def\csname faicon@stack-exchange\endcsname{{\FA\symbol{"F18D}}}
\expandafter\def\csname faicon@arrow-circle-o-right\endcsname{{\FA\symbol{"F18E}}}
\expandafter\def\csname faicon@arrow-circle-o-left\endcsname{{\FA\symbol{"F190}}}
\expandafter\def\csname faicon@caret-square-o-left\endcsname{{\FA\symbol{"F191}}}
\expandafter\def\csname faicon@dot-circle-o\endcsname{{\FA\symbol{"F192}}}
\expandafter\def\csname faicon@wheelchair\endcsname{{\FA\symbol{"F193}}}
\expandafter\def\csname faicon@vimeo-square\endcsname{{\FA\symbol{"F194}}}
\expandafter\def\csname faicon@try\endcsname{{\FA\symbol{"F195}}}
\expandafter\def\csname faicon@plus-square-o\endcsname{{\FA\symbol{"F196}}}
\expandafter\def\csname faicon@space-shuttle\endcsname{{\FA\symbol{"F197}}}
\expandafter\def\csname faicon@slack\endcsname{{\FA\symbol{"F198}}}
\expandafter\def\csname faicon@envelope-square\endcsname{{\FA\symbol{"F199}}}
\expandafter\def\csname faicon@wordpress\endcsname{{\FA\symbol{"F19A}}}
\expandafter\def\csname faicon@openid\endcsname{{\FA\symbol{"F19B}}}
\expandafter\def\csname faicon@university\endcsname{{\FA\symbol{"F19C}}}
\expandafter\def\csname faicon@graduation-cap\endcsname{{\FA\symbol{"F19D}}}
\expandafter\def\csname faicon@yahoo\endcsname{{\FA\symbol{"F19E}}}
\expandafter\def\csname faicon@google\endcsname{{\FA\symbol{"F1A0}}}
\expandafter\def\csname faicon@reddit\endcsname{{\FA\symbol{"F1A1}}}
\expandafter\def\csname faicon@reddit-square\endcsname{{\FA\symbol{"F1A2}}}
\expandafter\def\csname faicon@stumbleupon-circle\endcsname{{\FA\symbol{"F1A3}}}
\expandafter\def\csname faicon@stumbleupon\endcsname{{\FA\symbol{"F1A4}}}
\expandafter\def\csname faicon@delicious\endcsname{{\FA\symbol{"F1A5}}}
\expandafter\def\csname faicon@digg\endcsname{{\FA\symbol{"F1A6}}}
\expandafter\def\csname faicon@pied-piper-pp\endcsname{{\FA\symbol{"F1A7}}}
\expandafter\def\csname faicon@pied-piper-alt\endcsname{{\FA\symbol{"F1A8}}}
\expandafter\def\csname faicon@drupal\endcsname{{\FA\symbol{"F1A9}}}
\expandafter\def\csname faicon@joomla\endcsname{{\FA\symbol{"F1AA}}}
\expandafter\def\csname faicon@language\endcsname{{\FA\symbol{"F1AB}}}
\expandafter\def\csname faicon@fax\endcsname{{\FA\symbol{"F1AC}}}
\expandafter\def\csname faicon@building\endcsname{{\FA\symbol{"F1AD}}}
\expandafter\def\csname faicon@child\endcsname{{\FA\symbol{"F1AE}}}
\expandafter\def\csname faicon@paw\endcsname{{\FA\symbol{"F1B0}}}
\expandafter\def\csname faicon@spoon\endcsname{{\FA\symbol{"F1B1}}}
\expandafter\def\csname faicon@cube\endcsname{{\FA\symbol{"F1B2}}}
\expandafter\def\csname faicon@cubes\endcsname{{\FA\symbol{"F1B3}}}
\expandafter\def\csname faicon@behance\endcsname{{\FA\symbol{"F1B4}}}
\expandafter\def\csname faicon@behance-square\endcsname{{\FA\symbol{"F1B5}}}
\expandafter\def\csname faicon@steam\endcsname{{\FA\symbol{"F1B6}}}
\expandafter\def\csname faicon@steam-square\endcsname{{\FA\symbol{"F1B7}}}
\expandafter\def\csname faicon@recycle\endcsname{{\FA\symbol{"F1B8}}}
\expandafter\def\csname faicon@car\endcsname{{\FA\symbol{"F1B9}}}
\expandafter\def\csname faicon@taxi\endcsname{{\FA\symbol{"F1BA}}}
\expandafter\def\csname faicon@tree\endcsname{{\FA\symbol{"F1BB}}}
\expandafter\def\csname faicon@spotify\endcsname{{\FA\symbol{"F1BC}}}
\expandafter\def\csname faicon@deviantart\endcsname{{\FA\symbol{"F1BD}}}
\expandafter\def\csname faicon@soundcloud\endcsname{{\FA\symbol{"F1BE}}}
\expandafter\def\csname faicon@database\endcsname{{\FA\symbol{"F1C0}}}
\expandafter\def\csname faicon@file-pdf-o\endcsname{{\FA\symbol{"F1C1}}}
\expandafter\def\csname faicon@file-word-o\endcsname{{\FA\symbol{"F1C2}}}
\expandafter\def\csname faicon@file-excel-o\endcsname{{\FA\symbol{"F1C3}}}
\expandafter\def\csname faicon@file-powerpoint-o\endcsname{{\FA\symbol{"F1C4}}}
\expandafter\def\csname faicon@file-image-o\endcsname{{\FA\symbol{"F1C5}}}
\expandafter\def\csname faicon@file-archive-o\endcsname{{\FA\symbol{"F1C6}}}
\expandafter\def\csname faicon@file-audio-o\endcsname{{\FA\symbol{"F1C7}}}
\expandafter\def\csname faicon@file-video-o\endcsname{{\FA\symbol{"F1C8}}}
\expandafter\def\csname faicon@file-code-o\endcsname{{\FA\symbol{"F1C9}}}
\expandafter\def\csname faicon@vine\endcsname{{\FA\symbol{"F1CA}}}
\expandafter\def\csname faicon@codepen\endcsname{{\FA\symbol{"F1CB}}}
\expandafter\def\csname faicon@jsfiddle\endcsname{{\FA\symbol{"F1CC}}}
\expandafter\def\csname faicon@life-ring\endcsname{{\FA\symbol{"F1CD}}}
\expandafter\def\csname faicon@circle-o-notch\endcsname{{\FA\symbol{"F1CE}}}
\expandafter\def\csname faicon@rebel\endcsname{{\FA\symbol{"F1D0}}}
\expandafter\def\csname faicon@empire\endcsname{{\FA\symbol{"F1D1}}}
\expandafter\def\csname faicon@git-square\endcsname{{\FA\symbol{"F1D2}}}
\expandafter\def\csname faicon@git\endcsname{{\FA\symbol{"F1D3}}}
\expandafter\def\csname faicon@hacker-news\endcsname{{\FA\symbol{"F1D4}}}
\expandafter\def\csname faicon@tencent-weibo\endcsname{{\FA\symbol{"F1D5}}}
\expandafter\def\csname faicon@qq\endcsname{{\FA\symbol{"F1D6}}}
\expandafter\def\csname faicon@weixin\endcsname{{\FA\symbol{"F1D7}}}
\expandafter\def\csname faicon@paper-plane\endcsname{{\FA\symbol{"F1D8}}}
\expandafter\def\csname faicon@paper-plane-o\endcsname{{\FA\symbol{"F1D9}}}
\expandafter\def\csname faicon@history\endcsname{{\FA\symbol{"F1DA}}}
\expandafter\def\csname faicon@circle-thin\endcsname{{\FA\symbol{"F1DB}}}
\expandafter\def\csname faicon@header\endcsname{{\FA\symbol{"F1DC}}}
\expandafter\def\csname faicon@paragraph\endcsname{{\FA\symbol{"F1DD}}}
\expandafter\def\csname faicon@sliders\endcsname{{\FA\symbol{"F1DE}}}
\expandafter\def\csname faicon@share-alt\endcsname{{\FA\symbol{"F1E0}}}
\expandafter\def\csname faicon@share-alt-square\endcsname{{\FA\symbol{"F1E1}}}
\expandafter\def\csname faicon@bomb\endcsname{{\FA\symbol{"F1E2}}}
\expandafter\def\csname faicon@futbol-o\endcsname{{\FA\symbol{"F1E3}}}
\expandafter\def\csname faicon@tty\endcsname{{\FA\symbol{"F1E4}}}
\expandafter\def\csname faicon@binoculars\endcsname{{\FA\symbol{"F1E5}}}
\expandafter\def\csname faicon@plug\endcsname{{\FA\symbol{"F1E6}}}
\expandafter\def\csname faicon@slideshare\endcsname{{\FA\symbol{"F1E7}}}
\expandafter\def\csname faicon@twitch\endcsname{{\FA\symbol{"F1E8}}}
\expandafter\def\csname faicon@yelp\endcsname{{\FA\symbol{"F1E9}}}
\expandafter\def\csname faicon@newspaper-o\endcsname{{\FA\symbol{"F1EA}}}
\expandafter\def\csname faicon@wifi\endcsname{{\FA\symbol{"F1EB}}}
\expandafter\def\csname faicon@calculator\endcsname{{\FA\symbol{"F1EC}}}
\expandafter\def\csname faicon@paypal\endcsname{{\FA\symbol{"F1ED}}}
\expandafter\def\csname faicon@google-wallet\endcsname{{\FA\symbol{"F1EE}}}
\expandafter\def\csname faicon@cc-visa\endcsname{{\FA\symbol{"F1F0}}}
\expandafter\def\csname faicon@cc-mastercard\endcsname{{\FA\symbol{"F1F1}}}
\expandafter\def\csname faicon@cc-discover\endcsname{{\FA\symbol{"F1F2}}}
\expandafter\def\csname faicon@cc-amex\endcsname{{\FA\symbol{"F1F3}}}
\expandafter\def\csname faicon@cc-paypal\endcsname{{\FA\symbol{"F1F4}}}
\expandafter\def\csname faicon@cc-stripe\endcsname{{\FA\symbol{"F1F5}}}
\expandafter\def\csname faicon@bell-slash\endcsname{{\FA\symbol{"F1F6}}}
\expandafter\def\csname faicon@bell-slash-o\endcsname{{\FA\symbol{"F1F7}}}
\expandafter\def\csname faicon@trash\endcsname{{\FA\symbol{"F1F8}}}
\expandafter\def\csname faicon@copyright\endcsname{{\FA\symbol{"F1F9}}}
\expandafter\def\csname faicon@at\endcsname{{\FA\symbol{"F1FA}}}
\expandafter\def\csname faicon@eyedropper\endcsname{{\FA\symbol{"F1FB}}}
\expandafter\def\csname faicon@paint-brush\endcsname{{\FA\symbol{"F1FC}}}
\expandafter\def\csname faicon@birthday-cake\endcsname{{\FA\symbol{"F1FD}}}
\expandafter\def\csname faicon@area-chart\endcsname{{\FA\symbol{"F1FE}}}
\expandafter\def\csname faicon@pie-chart\endcsname{{\FA\symbol{"F200}}}
\expandafter\def\csname faicon@line-chart\endcsname{{\FA\symbol{"F201}}}
\expandafter\def\csname faicon@lastfm\endcsname{{\FA\symbol{"F202}}}
\expandafter\def\csname faicon@lastfm-square\endcsname{{\FA\symbol{"F203}}}
\expandafter\def\csname faicon@toggle-off\endcsname{{\FA\symbol{"F204}}}
\expandafter\def\csname faicon@toggle-on\endcsname{{\FA\symbol{"F205}}}
\expandafter\def\csname faicon@bicycle\endcsname{{\FA\symbol{"F206}}}
\expandafter\def\csname faicon@bus\endcsname{{\FA\symbol{"F207}}}
\expandafter\def\csname faicon@ioxhost\endcsname{{\FA\symbol{"F208}}}
\expandafter\def\csname faicon@angellist\endcsname{{\FA\symbol{"F209}}}
\expandafter\def\csname faicon@cc\endcsname{{\FA\symbol{"F20A}}}
\expandafter\def\csname faicon@ils\endcsname{{\FA\symbol{"F20B}}}
\expandafter\def\csname faicon@meanpath\endcsname{{\FA\symbol{"F20C}}}
\expandafter\def\csname faicon@buysellads\endcsname{{\FA\symbol{"F20D}}}
\expandafter\def\csname faicon@connectdevelop\endcsname{{\FA\symbol{"F20E}}}
\expandafter\def\csname faicon@dashcube\endcsname{{\FA\symbol{"F210}}}
\expandafter\def\csname faicon@forumbee\endcsname{{\FA\symbol{"F211}}}
\expandafter\def\csname faicon@leanpub\endcsname{{\FA\symbol{"F212}}}
\expandafter\def\csname faicon@sellsy\endcsname{{\FA\symbol{"F213}}}
\expandafter\def\csname faicon@shirtsinbulk\endcsname{{\FA\symbol{"F214}}}
\expandafter\def\csname faicon@simplybuilt\endcsname{{\FA\symbol{"F215}}}
\expandafter\def\csname faicon@skyatlas\endcsname{{\FA\symbol{"F216}}}
\expandafter\def\csname faicon@cart-plus\endcsname{{\FA\symbol{"F217}}}
\expandafter\def\csname faicon@cart-arrow-down\endcsname{{\FA\symbol{"F218}}}
\expandafter\def\csname faicon@diamond\endcsname{{\FA\symbol{"F219}}}
\expandafter\def\csname faicon@ship\endcsname{{\FA\symbol{"F21A}}}
\expandafter\def\csname faicon@user-secret\endcsname{{\FA\symbol{"F21B}}}
\expandafter\def\csname faicon@motorcycle\endcsname{{\FA\symbol{"F21C}}}
\expandafter\def\csname faicon@street-view\endcsname{{\FA\symbol{"F21D}}}
\expandafter\def\csname faicon@heartbeat\endcsname{{\FA\symbol{"F21E}}}
\expandafter\def\csname faicon@venus\endcsname{{\FA\symbol{"F221}}}
\expandafter\def\csname faicon@mars\endcsname{{\FA\symbol{"F222}}}
\expandafter\def\csname faicon@mercury\endcsname{{\FA\symbol{"F223}}}
\expandafter\def\csname faicon@transgender\endcsname{{\FA\symbol{"F224}}}
\expandafter\def\csname faicon@transgender-alt\endcsname{{\FA\symbol{"F225}}}
\expandafter\def\csname faicon@venus-double\endcsname{{\FA\symbol{"F226}}}
\expandafter\def\csname faicon@mars-double\endcsname{{\FA\symbol{"F227}}}
\expandafter\def\csname faicon@venus-mars\endcsname{{\FA\symbol{"F228}}}
\expandafter\def\csname faicon@mars-stroke\endcsname{{\FA\symbol{"F229}}}
\expandafter\def\csname faicon@mars-stroke-v\endcsname{{\FA\symbol{"F22A}}}
\expandafter\def\csname faicon@mars-stroke-h\endcsname{{\FA\symbol{"F22B}}}
\expandafter\def\csname faicon@neuter\endcsname{{\FA\symbol{"F22C}}}
\expandafter\def\csname faicon@genderless\endcsname{{\FA\symbol{"F22D}}}
\expandafter\def\csname faicon@facebook-official\endcsname{{\FA\symbol{"F230}}}
\expandafter\def\csname faicon@pinterest-p\endcsname{{\FA\symbol{"F231}}}
\expandafter\def\csname faicon@whatsapp\endcsname{{\FA\symbol{"F232}}}
\expandafter\def\csname faicon@server\endcsname{{\FA\symbol{"F233}}}
\expandafter\def\csname faicon@user-plus\endcsname{{\FA\symbol{"F234}}}
\expandafter\def\csname faicon@user-times\endcsname{{\FA\symbol{"F235}}}
\expandafter\def\csname faicon@bed\endcsname{{\FA\symbol{"F236}}}
\expandafter\def\csname faicon@viacoin\endcsname{{\FA\symbol{"F237}}}
\expandafter\def\csname faicon@train\endcsname{{\FA\symbol{"F238}}}
\expandafter\def\csname faicon@subway\endcsname{{\FA\symbol{"F239}}}
\expandafter\def\csname faicon@medium\endcsname{{\FA\symbol{"F23A}}}
\expandafter\def\csname faicon@y-combinator\endcsname{{\FA\symbol{"F23B}}}
\expandafter\def\csname faicon@optin-monster\endcsname{{\FA\symbol{"F23C}}}
\expandafter\def\csname faicon@opencart\endcsname{{\FA\symbol{"F23D}}}
\expandafter\def\csname faicon@expeditedssl\endcsname{{\FA\symbol{"F23E}}}
\expandafter\def\csname faicon@battery-full\endcsname{{\FA\symbol{"F240}}}
\expandafter\def\csname faicon@battery-three-quarters\endcsname{{\FA\symbol{"F241}}}
\expandafter\def\csname faicon@battery-half\endcsname{{\FA\symbol{"F242}}}
\expandafter\def\csname faicon@battery-quarter\endcsname{{\FA\symbol{"F243}}}
\expandafter\def\csname faicon@battery-empty\endcsname{{\FA\symbol{"F244}}}
\expandafter\def\csname faicon@mouse-pointer\endcsname{{\FA\symbol{"F245}}}
\expandafter\def\csname faicon@i-cursor\endcsname{{\FA\symbol{"F246}}}
\expandafter\def\csname faicon@object-group\endcsname{{\FA\symbol{"F247}}}
\expandafter\def\csname faicon@object-ungroup\endcsname{{\FA\symbol{"F248}}}
\expandafter\def\csname faicon@sticky-note\endcsname{{\FA\symbol{"F249}}}
\expandafter\def\csname faicon@sticky-note-o\endcsname{{\FA\symbol{"F24A}}}
\expandafter\def\csname faicon@cc-jcb\endcsname{{\FA\symbol{"F24B}}}
\expandafter\def\csname faicon@cc-diners-club\endcsname{{\FA\symbol{"F24C}}}
\expandafter\def\csname faicon@clone\endcsname{{\FA\symbol{"F24D}}}
\expandafter\def\csname faicon@balance-scale\endcsname{{\FA\symbol{"F24E}}}
\expandafter\def\csname faicon@hourglass-o\endcsname{{\FA\symbol{"F250}}}
\expandafter\def\csname faicon@hourglass-start\endcsname{{\FA\symbol{"F251}}}
\expandafter\def\csname faicon@hourglass-half\endcsname{{\FA\symbol{"F252}}}
\expandafter\def\csname faicon@hourglass-end\endcsname{{\FA\symbol{"F253}}}
\expandafter\def\csname faicon@hourglass\endcsname{{\FA\symbol{"F254}}}
\expandafter\def\csname faicon@hand-rock-o\endcsname{{\FA\symbol{"F255}}}
\expandafter\def\csname faicon@hand-paper-o\endcsname{{\FA\symbol{"F256}}}
\expandafter\def\csname faicon@hand-scissors-o\endcsname{{\FA\symbol{"F257}}}
\expandafter\def\csname faicon@hand-lizard-o\endcsname{{\FA\symbol{"F258}}}
\expandafter\def\csname faicon@hand-spock-o\endcsname{{\FA\symbol{"F259}}}
\expandafter\def\csname faicon@hand-pointer-o\endcsname{{\FA\symbol{"F25A}}}
\expandafter\def\csname faicon@hand-peace-o\endcsname{{\FA\symbol{"F25B}}}
\expandafter\def\csname faicon@trademark\endcsname{{\FA\symbol{"F25C}}}
\expandafter\def\csname faicon@registered\endcsname{{\FA\symbol{"F25D}}}
\expandafter\def\csname faicon@creative-commons\endcsname{{\FA\symbol{"F25E}}}
\expandafter\def\csname faicon@gg\endcsname{{\FA\symbol{"F260}}}
\expandafter\def\csname faicon@gg-circle\endcsname{{\FA\symbol{"F261}}}
\expandafter\def\csname faicon@tripadvisor\endcsname{{\FA\symbol{"F262}}}
\expandafter\def\csname faicon@odnoklassniki\endcsname{{\FA\symbol{"F263}}}
\expandafter\def\csname faicon@odnoklassniki-square\endcsname{{\FA\symbol{"F264}}}
\expandafter\def\csname faicon@get-pocket\endcsname{{\FA\symbol{"F265}}}
\expandafter\def\csname faicon@wikipedia-w\endcsname{{\FA\symbol{"F266}}}
\expandafter\def\csname faicon@safari\endcsname{{\FA\symbol{"F267}}}
\expandafter\def\csname faicon@chrome\endcsname{{\FA\symbol{"F268}}}
\expandafter\def\csname faicon@firefox\endcsname{{\FA\symbol{"F269}}}
\expandafter\def\csname faicon@opera\endcsname{{\FA\symbol{"F26A}}}
\expandafter\def\csname faicon@internet-explorer\endcsname{{\FA\symbol{"F26B}}}
\expandafter\def\csname faicon@television\endcsname{{\FA\symbol{"F26C}}}
\expandafter\def\csname faicon@contao\endcsname{{\FA\symbol{"F26D}}}
\expandafter\def\csname faicon@500px\endcsname{{\FA\symbol{"F26E}}}
\expandafter\def\csname faicon@amazon\endcsname{{\FA\symbol{"F270}}}
\expandafter\def\csname faicon@calendar-plus-o\endcsname{{\FA\symbol{"F271}}}
\expandafter\def\csname faicon@calendar-minus-o\endcsname{{\FA\symbol{"F272}}}
\expandafter\def\csname faicon@calendar-times-o\endcsname{{\FA\symbol{"F273}}}
\expandafter\def\csname faicon@calendar-check-o\endcsname{{\FA\symbol{"F274}}}
\expandafter\def\csname faicon@industry\endcsname{{\FA\symbol{"F275}}}
\expandafter\def\csname faicon@map-pin\endcsname{{\FA\symbol{"F276}}}
\expandafter\def\csname faicon@map-signs\endcsname{{\FA\symbol{"F277}}}
\expandafter\def\csname faicon@map-o\endcsname{{\FA\symbol{"F278}}}
\expandafter\def\csname faicon@map\endcsname{{\FA\symbol{"F279}}}
\expandafter\def\csname faicon@commenting\endcsname{{\FA\symbol{"F27A}}}
\expandafter\def\csname faicon@commenting-o\endcsname{{\FA\symbol{"F27B}}}
\expandafter\def\csname faicon@houzz\endcsname{{\FA\symbol{"F27C}}}
\expandafter\def\csname faicon@vimeo\endcsname{{\FA\symbol{"F27D}}}
\expandafter\def\csname faicon@black-tie\endcsname{{\FA\symbol{"F27E}}}
\expandafter\def\csname faicon@fonticons\endcsname{{\FA\symbol{"F280}}}
\expandafter\def\csname faicon@reddit-alien\endcsname{{\FA\symbol{"F281}}}
\expandafter\def\csname faicon@edge\endcsname{{\FA\symbol{"F282}}}
\expandafter\def\csname faicon@credit-card-alt\endcsname{{\FA\symbol{"F283}}}
\expandafter\def\csname faicon@codiepie\endcsname{{\FA\symbol{"F284}}}
\expandafter\def\csname faicon@modx\endcsname{{\FA\symbol{"F285}}}
\expandafter\def\csname faicon@fort-awesome\endcsname{{\FA\symbol{"F286}}}
\expandafter\def\csname faicon@usb\endcsname{{\FA\symbol{"F287}}}
\expandafter\def\csname faicon@product-hunt\endcsname{{\FA\symbol{"F288}}}
\expandafter\def\csname faicon@mixcloud\endcsname{{\FA\symbol{"F289}}}
\expandafter\def\csname faicon@scribd\endcsname{{\FA\symbol{"F28A}}}
\expandafter\def\csname faicon@pause-circle\endcsname{{\FA\symbol{"F28B}}}
\expandafter\def\csname faicon@pause-circle-o\endcsname{{\FA\symbol{"F28C}}}
\expandafter\def\csname faicon@stop-circle\endcsname{{\FA\symbol{"F28D}}}
\expandafter\def\csname faicon@stop-circle-o\endcsname{{\FA\symbol{"F28E}}}
\expandafter\def\csname faicon@shopping-bag\endcsname{{\FA\symbol{"F290}}}
\expandafter\def\csname faicon@shopping-basket\endcsname{{\FA\symbol{"F291}}}
\expandafter\def\csname faicon@hashtag\endcsname{{\FA\symbol{"F292}}}
\expandafter\def\csname faicon@bluetooth\endcsname{{\FA\symbol{"F293}}}
\expandafter\def\csname faicon@bluetooth-b\endcsname{{\FA\symbol{"F294}}}
\expandafter\def\csname faicon@percent\endcsname{{\FA\symbol{"F295}}}
\expandafter\def\csname faicon@gitlab\endcsname{{\FA\symbol{"F296}}}
\expandafter\def\csname faicon@wpbeginner\endcsname{{\FA\symbol{"F297}}}
\expandafter\def\csname faicon@wpforms\endcsname{{\FA\symbol{"F298}}}
\expandafter\def\csname faicon@envira\endcsname{{\FA\symbol{"F299}}}
\expandafter\def\csname faicon@universal-access\endcsname{{\FA\symbol{"F29A}}}
\expandafter\def\csname faicon@wheelchair-alt\endcsname{{\FA\symbol{"F29B}}}
\expandafter\def\csname faicon@question-circle-o\endcsname{{\FA\symbol{"F29C}}}
\expandafter\def\csname faicon@blind\endcsname{{\FA\symbol{"F29D}}}
\expandafter\def\csname faicon@audio-description\endcsname{{\FA\symbol{"F29E}}}
\expandafter\def\csname faicon@volume-control-phone\endcsname{{\FA\symbol{"F2A0}}}
\expandafter\def\csname faicon@braille\endcsname{{\FA\symbol{"F2A1}}}
\expandafter\def\csname faicon@assistive-listening-systems\endcsname{{\FA\symbol{"F2A2}}}
\expandafter\def\csname faicon@american-sign-language-interpreting\endcsname{{\FA\symbol{"F2A3}}}
\expandafter\def\csname faicon@deaf\endcsname{{\FA\symbol{"F2A4}}}
\expandafter\def\csname faicon@glide\endcsname{{\FA\symbol{"F2A5}}}
\expandafter\def\csname faicon@glide-g\endcsname{{\FA\symbol{"F2A6}}}
\expandafter\def\csname faicon@sign-language\endcsname{{\FA\symbol{"F2A7}}}
\expandafter\def\csname faicon@low-vision\endcsname{{\FA\symbol{"F2A8}}}
\expandafter\def\csname faicon@viadeo\endcsname{{\FA\symbol{"F2A9}}}
\expandafter\def\csname faicon@viadeo-square\endcsname{{\FA\symbol{"F2AA}}}
\expandafter\def\csname faicon@snapchat\endcsname{{\FA\symbol{"F2AB}}}
\expandafter\def\csname faicon@snapchat-ghost\endcsname{{\FA\symbol{"F2AC}}}
\expandafter\def\csname faicon@snapchat-square\endcsname{{\FA\symbol{"F2AD}}}
\expandafter\def\csname faicon@pied-piper\endcsname{{\FA\symbol{"F2AE}}}
\expandafter\def\csname faicon@first-order\endcsname{{\FA\symbol{"F2B0}}}
\expandafter\def\csname faicon@yoast\endcsname{{\FA\symbol{"F2B1}}}
\expandafter\def\csname faicon@themeisle\endcsname{{\FA\symbol{"F2B2}}}
\expandafter\def\csname faicon@google-plus-official\endcsname{{\FA\symbol{"F2B3}}}
\expandafter\def\csname faicon@font-awesome\endcsname{{\FA\symbol{"F2B4}}}


==> implem.tex <==


We have implemented {\sc Code2Que} as a standalone web-based tool to assist developers in improving question titles in Stack Overflow.
The source code and data can be found in our Github repository\footnote{\url{https://github.com/beyondacm/Code2Que}}.

\smallskip
\noindent{\itshape\bfseries Data Collection}.
The data source of {\sc Code2Que} is from the Stack Overflow data dump of September 2019\footnote{\url{https://archive.org/details/stackexchange}}. We use the \textit{Python}, \textit{Java}, \textit{Javascript}, \textit{C\#} and \textit{SQL} tags to collect questions associated with the corresponding programming language. We extract the code snippet from each post's body by using $\langle$\textit{code}$\rangle$ tags, and then pair it with its question title if the question score is higher than 1. 
We have collected more than 1 million $\langle$\textit{code snippet}, \textit{question}$\rangle$ pairs from Stack Overflow for different programming languages.

\smallskip
\noindent{\itshape\bfseries Data Preprocessing}.
We preprocess our collected data according to the following steps: We first tokenize the code snippet and question title using the NLTK toolkit~\cite{bird2004nltk} (Step1). After that, to  avoid being overly context-specific, we use regular expressions to replace numbers and strings with special tokens ``NUMBER'' and ``STRING'' in code snippets (Step2). 
For question titles, we only keep the pairs if one of the interrogative keywords (e.g., ``how'', ``what'', ``why'', ``which'') appears in the question (Step3). Following that, we remove pairs where the code snippet and the question title are too long or too short. We set the token range from 16 tokens to 128 tokens for code snippets and from 4 tokens to 16 tokens for question titles respectively.  
The remaining $\langle$\textit{code snippet}, \textit{question}$\rangle$ pairs are added to our training corpus.

\begin{figure}[t]
    \centerline{\includegraphics[width=0.35\textwidth]{homepage-02.png}}
\vspace*{-10pt}
\caption{Homepage of Code2Que}
\vspace*{-0.5cm}
\label{fig:homepage}
\end{figure}

\smallskip
\noindent{\itshape\bfseries Backend Model}.
We use the framework OpenNMT~\cite{opennmt} to train our backend Model. 
We followed our previous experiment settings ~\cite{gao2020generating} for the training process.
The collected $\langle$\textit{question}, \textit{code snippet}$\rangle$ pairs are input into the workflow of our approach described in Section ~\ref{sec:approach}, and the output consists of the trained sequence-to-sequence model and the associated code embeddings which are used by {\sc Code2Que} as the backend model for online recommendation.

\smallskip
\noindent{\itshape\bfseries Frontend User Interface}.
%\subsection{Frontend User Interface}
Fig.~\ref{fig:homepage} shows the query page of {\sc Code2Que}.
{\sc Code2Que} provides an input box for developers to submit their source code snippet. After a developer submits his/her code snippet to the server, the code snippet is preprocessed and passed to our backend model. The outputs are organised into two separate result boxes for the generated question and retrieved questions respectively. For the generated question, {\sc Code2Que} generates a question title according to the code snippet.  For retrieved questions, {\sc Code2Que} returns the top-5 most similar questions in our code base together with the links to their Stack Overflow posts. 

\smallskip
\noindent{\itshape\bfseries System Optimization}.
To meet the efficiency requirement as an online web tool, we optimize the implementations of {\sc Code2Que}: 
(i) Considering that the offline learning model and code embeddings are frequently used in the online recommendation phase, we put them into cache to reduce redundant data loading. (ii) We created an index for the relevant questions in our database to speed up retrieval. (iii) We used locality sensitive hashing for fast nearest neighbour search in our large code embeddings data sets.




% \begin{figure}[t]
%     \centerline{\includegraphics[width=0.43\textwidth]{tool-bug-detection-print.pdf}}
% \vspace*{-10pt}
% \caption{Sample Results of Bug Detection}\vspace*{-0.6cm}
% \label{fig:tool-bug}
% \end{figure}

==> ref.tex <==
% comment is important 
% what is todo comment 
% what is the problem with todo comment 
% challeges 
% previous work 

% Ex1. https://github.com/expectocode/telegram-export/commit/d03bc0f2147658779ce14820608a8ba09d36e434
% Ex2. https://github.com/pyelasticsearch/pyelasticsearch/commit/a3f57d729b8631e7b6c2fe55e10455f2bcc4b581
% Ex3. https://github.com/Scifabric/pybossa/commit/3264aceb725268775e8659a6e6c9129d6a585939
% Ex3. https://github.com/21dotco/two1-python/commit/57ee38740060fc4cefa0a5be73e835ae866b0658
% Ex4. https://github.com/expectocode/telegram-export/commit/5cc109a9eedaaefe3cb21bff1b0bb6edc46c08a1
% Ex5. https://github.com/expectocode/telegram-export/commit/402c48294e7effa76ceac1e57374ecf03066e1ec
% Ex6. https://github.com/pfultz2/cget/commit/38403914ce74ae2a5c36a9271d802f0b2bf2cdd4
% Ex7. https://github.com/pyelasticsearch/pyelasticsearch/commit/cb0b7e9431f5cb8c9f5fe8a2f5033aad23d2fc01
% Ex8. https://github.com/pyelasticsearch/pyelasticsearch/commit/a3f57d729b8631e7b6c2fe55e10455f2bcc4b581
% Ex9. https://github.com/Scifabric/pybossa/commit/d006276e39ef0800bba9775e125ca4cdd08e49b7

% Motivation Examples:
% https://github.com/Shmuma/ptan/commit/66290f1c7150948ce20d7a02302b9072abd2a732
% https://github.com/coderholic/pyradio/commit/714d8a565f928363f6bbe655967d4b45f4a8f053 *
% https://github.com/21dotco/two1-python/commit/9cefc94e6b190ec3b23d913fe6189890ac4ec443 * 
% https://github.com/21dotco/two1-python/commit/3e54ba6bac35a5f86f68ff17d3f3823cb3d1521b 
% https://github.com/21dotco/two1-python/commit/89981585fcbb15d1ade2ce0f8019f6ae581bf964
% https://github.com/expectocode/telegram-export/commit/0096d4bf10af2d1ddc3c77922f13465d8affcceb
% https://github.com/pfultz2/cget/commit/4b303b2d043302a2425c223f92a6a870da140144
% https://github.com/tarmstrong/nbdiff/commit/d1373b6fbc37956ff41bd0a4afcb5e75bc21068f
% https://github.com/carefree0910/carefree-learn/commit/dc6fb7b141ca7e0efee5b5714d5c10bf845c18c6 * 
% https://github.com/concurrencylabs/aws-pricing-tools/commit/c6fa9c90949f5484d65899e2022af47262924a95
% https://github.com/inasafe/inasafe/commit/ac93e7f74784aca456868abe89f11ef9b9c267a6
% https://github.com/inasafe/inasafe/commit/7401878ecfbcf3f8050b7620a22b8816d8fd3a6b
% https://github.com/PaulSec/HQLmap/commit/25e07e122c06b1d9860f0734c686854709b85748
% https://github.com/homebysix/recipe-robot/commit/c4dc8c24e035b298bf867c60f07afbc8d0ea8e0a * 
% https://github.com/facebookresearch/ParlAI/commit/566c34205d5e5ff5f2315c612de6215ae79494ee
% https://github.com/iambus/xunlei-lixian/commit/6f6848617325fb3a44e13ab06855acf11bd24e85
% https://github.com/Kozea/WeasyPrint/commit/5a75887a83848fd471f745fa7b9fe224e0abe68d
% https://github.com/LibreScanner/horus/commit/17846848ff88fca25d90aeb1a7288be2e852f40e
% https://github.com/gorakhargosh/watchdog/commit/a9cafbbd1fb6943201cc6070dd072779612ce4ff **  
% https://github.com/jwlodek/py_cui/commit/5aa3e34162bde2d221c1595bb4a2f0463aebc392 
% https://github.com/dexy/dexy/commit/b59c53c70cd7e1081f11ad191e6fb1712e789a0e
% https://github.com/karlicoss/HPI/commit/c0bbb4eaf2365b43422691718efed64ebdef73c6
% https://github.com/conda-forge/staged-recipes/commit/f84bcd0c528607637c3ceafd865320e69ede129d ** 
% https://github.com/faucetsdn/faucet/commit/65d95d97df7870bd6faf12f569f9389f3d214c33 * 
% https://github.com/matrix-org/synapse/commit/806f380a8b448ce03671f1ce07f7dfcbdc5261e1 * 
% https://github.com/Trusted-AI/adversarial-robustness-toolbox/commit/a335b22ef1eff3eb50aac20d22fd4f80f7c2a912 
% https://github.com/more-itertools/more-itertools/commit/59d3ac2cb8ea91ade585b1131c9c819f0530a359
% https://github.com/ansible/ansible/commit/db83c0e7cdac8e86026eeae5314185c667e6da1c * 
% https://github.com/kpreid/shinysdr/commit/bfa746a501f8ff0e585199ae35d20fd46a1858e2 
% https://github.com/pyscf/pyscf/commit/881478b155984f96eff6850171fab510dca5d26c
% https://github.com/SublimeHaskell/SublimeHaskell/commit/f52236c89ae82d3fbcda5eb0a72ec0a1999a49bb * 
% https://github.com/openstack/nova/commit/e8a2a540e574ca2d242b9c2749c1f285498809e7 ***
% https://github.com/conan-io/conan-center-index/commit/ea6996cf915d5a769296817c0e2f9f73496a04ca
% https://github.com/cupy/cupy/commit/f76269726d70d0aae83555c6266973dafc0aec1e
% https://github.com/matplotlib/matplotlib/commit/6a6f8d9fcc9f93fc209f289d851350e29a82764d ***
% https://github.com/google/TensorNetwork/commit/50849ce792a1dcdf2a445af83125d06a5c25df09
% https://github.com/torrvision/crayon/commit/2e3641505174241f9f478e3d17d645c830d41297
% https://github.com/oppia/oppia/commit/a43d4d4c618f48b49622502387dc48c309219228 * 
% https://github.com/zulip/zulip/commit/478e215acd6552fc994bd82c9d78f68b7df627d5
% https://github.com/bridgecrewio/checkov/commit/fb95ac4f6eca2f2267d56e469b1fe3544eed66ea *
% https://github.com/google/jax/commit/bd14f2343aece428df85808d23cace1ede0b2821
% https://github.com/certbot/certbot/commit/7feab30e72f5b2fa6fbf23017cafdfb474b5ab72
% https://github.com/joeyespo/grip/commit/a66ce7e8048d6d108fc1bf6d8d7c12a83e77059
% https://github.com/pantsbuild/pants/commit/4f2db5291cbdb1a9d1dd1f847859725f14a19edd
% https://github.com/Trusted-AI/adversarial-robustness-toolbox/commit/4408c3e800513a4e7b83cf794d5c9af04d838d3c
% https://github.com/johnnykv/heralding/commit/d168b7e6c449cb0c2824a51c6bac98af2485b07e
% https://github.com/MagicStack/httptools/commit/44050b4dab8a7d93f878fe2964b2aa496f1151a6
% https://github.com/priba/nmp_qc/commit/77cf5a108a2c38509d988bf676131498a4f89f8b
% https://github.com/HyperGAN/HyperGAN/commit/20632411876bebb6d1a91a6347fa9f1f78ca47ea
% https://github.com/uma-pi1/kge/commit/2fa6ba193212f79e461843ba008885d648078d97 * 
% https://github.com/asyml/texar/commit/c0796197d5629f53c065477071bb2e4700230544
% https://github.com/mdn/kuma/commit/68a90af2f1397890700ace7a6954420a6cc2a587
% https://github.com/LonamiWebs/Telethon/commit/795cb989099a940a1bd065f8212f5fe650c2bf18
% https://github.com/ethereum/trinity/commit/f172b7a3671df75bf9faa9fbce16f2a0a72c3499 **
% https://github.com/drscotthawley/panotti/commit/073349264d61750b83d35a7ca1907cd0bfa4291c
% https://github.com/great-expectations/great_expectations/commit/8ad46babfeaeef7482aa8e7f42260ba0559a5d49 * 
% https://github.com/python/mypy/commit/a8d52612f781f72ffb5facca2ab8233705bc343d * 
% https://github.com/ICSec/airpwn-ng/commit/2aaeacaaf3d0e251f31c59250f79a0c616fde3bf 
% https://github.com/freenas/freenas/commit/265c92eb77d389e4590a558ba5cc9d4330b4b7ca * 
% https://github.com/aws/chalice/commit/f24e7520212a9c36a0ce4dbde483e9cb64193f31 * 
% https://github.com/cowrie/cowrie/commit/ee177d5482bed7a8908f742e26bb334408df328e * 
% https://github.com/google/clusterfuzz/commit/055b529c4c8958711c0530637fa901e1b935d53a ****  
% https://github.com/openid/python-openid/commit/3b015fb69b956d4b2bd5d7010d89daaf126e8be8 * 
% https://github.com/rootzoll/raspiblitz/commit/26cad6c6ef5cf908cd9d6bfea5d7e43c1fe2a546
% https://github.com/faucetsdn/faucet/commit/d63df4657883fefcbc43d0d3706a05316853d996
% https://github.com/dimagi/commcare-hq/commit/1f4809db8a98d775c4f7a4d3a032e0960aef38f6 * 
% https://github.com/Fuyukai/Kyoukai/commit/4b53baf7a364256940c7a96170e6c6cf1c63f6af 
% https://github.com/rhinstaller/anaconda/commit/711cbaf3ce41bd8dab899ab76fd3efbb89933b37 * 
% https://github.com/tribe29/checkmk/commit/f2115724f29ece525e88ce7005324e17953e0737 * 

% User Study Examples
% https://github.com/carefree0910/carefree-learn/commit/dc6fb7b141ca7e0efee5b5714d5c10bf845c18c6
% https://github.com/ansible/ansible/commit/db83c0e7cdac8e86026eeae5314185c667e6da1c
% https://github.com/bridgecrewio/checkov/commit/fb95ac4f6eca2f2267d56e469b1fe3544eed66ea (resolved)
% https://github.com/MagicStack/httptools/commit/44050b4dab8a7d93f878fe2964b2aa496f1151a6
% https://github.com/uma-pi1/kge/commit/2fa6ba193212f79e461843ba008885d648078d97
% https://github.com/drscotthawley/panotti/commit/073349264d61750b83d35a7ca1907cd0bfa4291c
% https://github.com/turicas/rows/commit/063eff251c5e013589454672af75c21492693fd2
% https://github.com/thonny/thonny/commit/2ef4d21da1f862f4e1ea464de05f8992bd61e09f
% https://github.com/dcos/dcos/commit/3dc98580365b70d0dd0fd2f29589384e0e922d87
% https://github.com/ctpbee/ctpbee/blob/master/ctpbee/constant.py
% https://github.com/openstack/nova/commit/f86f7ab64360d2294a855f9e770dfd6ac87832e5
% https://github.com/scipy/scipy/commit/0ca705543cda72346f16ff620a4295ae6974243b
% https://github.com/mozilla/MozDef/commit/b8f9aa8d10f0d854c20d1b7805043eed8249008e
% https://github.com/FasterXML/jackson-databind/commit/659408c3f5a0cf7d5cd9e5079ffa1ed828848f2a
% https://github.com/apache/flink/blob/master/flink-streaming-java/src/main/java/org/apache/flink/streaming/runtime/tasks/StreamTask.java
% https://github.com/grpc/grpc-java/commit/bb0c0e53c2e823154e153c240368e078d846af45
% https://github.com/LMAX-Exchange/disruptor/commit/85905a0f48db8a0997eb1a5c0bf5ec878d399345
% 

%undel 
% https://github.com/yt-project/yt/commit/1fcddfcdf042036e848d27bf5510c4cd41d370e2
% https://github.com/Azure/azure-cli/commit/6f28feb63eae5d9d9764ed98381f2f516dbcd66d
% https://github.com/milesrichardson/ParsePy/commit/7f651474398fc77de4313a0b8668401ab2fb7119
% https://github.com/netenglabs/suzieq/blob/master/tests/utilities/update_sqcmds.py
% https://github.com/netenglabs/suzieq/commit/ea68fd9f0fba9973b2b8d700c7d6087de77f3741
% 

% \subsection{Qualitative Analysis}
% https://github.com/pyelasticsearch/pyelasticsearch/commit/a3f57d729b8631e7b6c2fe55e10455f2bcc4b581
% https://github.com/1200wd/bitcoinlib/commit/307660c6f9521324cb75fa11c04654439aa40da8
% https://github.com/inasafe/inasafe/commit/5ca100c6752b53e6bad1f9af8f0d7a1e466b71f5 (introduction)
% https://github.com/1200wd/bitcoinlib/commit/355c1e1c513d39a00c229edda18809d266deebb3
% https://github.com/trufont/trufont/commit/ab1e70f2b2543c60259b7be127f70d062c51d0cb
% https://github.com/trufont/trufont/commit/772a09ae5e0b03595be92e9313223134cbcdfe4b
% https://github.com/imagej/imagej/commit/bb2e21c3fb7bf5539baa8bc6acfeb43f8429bccc
% https://github.com/imagej/imagej/commit/f14486df058a95bde62241f80c599ed880010b3c
% https://github.com/imagej/imagej/commit/473dd7e544aad9cb716fb0a6d5f57fa4676d30fa
% https://github.com/imagej/imagej/commit/4699b04efeda49273820815b5d506a33f4ed654d
% https://github.com/spring-projects/spring-batch/commit/d60c726121cd8906c71c5c7e5ade83310816f259
% https://github.com/spring-projects/spring-batch/commit/459f7d575db7b4899ab28336775c511d1e6938d9
% https://github.com/spring-projects/spring-batch/commit/394de964e1f6647309c3b6da7f280929584b0fe0
% https://github.com/spring-projects/spring-batch/commit/843ecf40d20c1a30a465e7b1c10d514824c5860f ****
% https://github.com/AndlyticsProject/andlytics/commit/90cd58c860039c6f463237abcf82867ccdb301e3
% https://github.com/davidmoten/rxjava2-jdbc/commit/65d12c09cffaaf0f5d44cc4907e9c50e16780e2c *** (introduction
% https://github.com/haiwen/seadroid/commit/ffcb11b113dc3a4ca0863df70d14d8764c5fb2be)
% https://github.com/imagej/imagej/commit/f2e46c27441db906788155b687e6f8cde3f2b7b3
% https://github.com/imagej/imagej/commit/844df0e1f36fde635531af7a4a908ad7e60f24c7
% https://github.com/imagej/imagej/commit/6bad6a89acedd2ee695d811a3b29b45f30f28660
% https://github.com/21dotco/two1-python/commit/3e54ba6bac35a5f86f68ff17d3f3823cb3d1521b ***

% https://github.com/pyelasticsearch/pyelasticsearch/commit/ecdd1900e9311eab2f32a431f97df8ea66e6080e
% https://github.com/pyelasticsearch/pyelasticsearch/commit/a3f57d729b8631e7b6c2fe55e10455f2bcc4b581
% https://github.com/Scifabric/pybossa/commit/af7530291f745f715fc445e177faf2afb8dc0633
% drop: https://github.com/Scifabric/pybossa/commit/7845f058c599ce7e26c6b14f3f601041cc24de79
% https://github.com/Games-and-Simulations/sc-docker/commit/33da40b1aab0dc23df7483ab7f0f6efd62eb8757
% https://github.com/timdouglas/sublime-less2css/commit/90f08ea5648d21b8c26971038bfa1fa45a4cc78d
% ??? : https://github.com/carefree0910/carefree-learn/commit/255bf8b754b1b61a2a873c080d0b1788879eca79 
% https://github.com/1200wd/bitcoinlib/commit/5fdbb8f900671fc86d2715027b4017e3b1e5cee5
% case study: https://github.com/1200wd/bitcoinlib/commit/7220d86a2f752594215555064d9dabada7f7e16a
% https://github.com/1200wd/bitcoinlib/commit/0823e9934c405c1233a322aaaf22f3f655eb32b9
% https://github.com/1200wd/bitcoinlib/commit/93d9292b25704a34e5ccf7f2c0d561d391bda2f5
% case study: https://github.com/1200wd/bitcoinlib/commit/f7915de68a0d7401c32f1fa6211f95664e6390d5
% https://github.com/1200wd/bitcoinlib/commit/f5585da0537ec97cb0b2b005fdcf9ed3913face3
% https://github.com/1200wd/bitcoinlib/commit/81948a4dfcb027e88ade92885bb8a180edb52868
% https://github.com/1200wd/bitcoinlib/commit/df11967a000074310f0acb6412ca37cb9189c0b6
% https://github.com/1200wd/bitcoinlib/commit/92fdb13082624e13536d125bd31c8728adcf1995
% https://github.com/1200wd/bitcoinlib/commit/f446fcd660551f0104cf920533526e17b3e32942
% https://github.com/1200wd/bitcoinlib/commit/307660c6f9521324cb75fa11c04654439aa40da8
% https://github.com/1200wd/bitcoinlib/commit/ac62287328336dacc4124c333547e949b92e20e1
% https://github.com/1200wd/bitcoinlib/commit/2edc7fabdc4701328798dc338da4dbeababae765
% https://github.com/webcompat/webcompat.com/commit/c47bcd9b23a1435e31ab49cad0076f5c6181cc7f
% https://github.com/webcompat/webcompat.com/commit/90f5b05945b3b501da6ffcd8301f9342d3bd7f4b
% https://github.com/webcompat/webcompat.com/commit/8457d9ee32bfd9705753f93e9c25dff61351c328
% https://github.com/webcompat/webcompat.com/commit/1a434ffa2cba09b594ac9bda0e1120927da6909b
% https://github.com/webcompat/webcompat.com/commit/eb0cf1c65e10d701308795955eba81e0c403c448
% https://github.com/aromanovich/jsl/commit/a28bee7d057c58810e84b1ea0072f8be2e5ece50
% https://github.com/wordnik/wordnik-python/commit/d0b4fdd9ef61b33a01eff250faee585f5180bb18
% https://github.com/inasafe/inasafe/commit/0227aeaa55c908dd6d81186c3da11baa61fefc6f
% case study: https://github.com/inasafe/inasafe/commit/5ca100c6752b53e6bad1f9af8f0d7a1e466b71f5
% https://github.com/mozilla/foundation.mozilla.org/commit/4ba7516ce7dc74932d40e3ee4d7048a7d4ce1f5c

% Java
% https://github.com/imagej/imagej/commit/ccd67d8d5a55d5674813055a7960fea4bef60b7d
% https://github.com/imagej/imagej/commit/d152ca154cd97067b38bd7a7779c6023e0247d98
% case study: https://github.com/imagej/imagej/commit/8513b489511ff3489b8ccba357b524c5f30d2b6c
% https://github.com/imagej/imagej/commit/a565c5550d0f992b3de0109bf968610a1885f753
% https://github.com/imagej/imagej/commit/3fbd192033119dbe41635e734416d90d26c5bbd2
% https://github.com/imagej/imagej/commit/1777d31b29a554d9b06375afebaab51c6d22e2a0
% https://github.com/shiffman/Most-Pixels-Ever-Processing/commit/2618da39b120e3cce7240d9eb88a63decb4359f4
% case study: https://github.com/marverenic/Jockey/commit/3b7c6b5feb38dffcfabf03f25ffbfff0371e0fe4
% https://github.com/marverenic/Jockey/commit/93d7a9692aec6e6af847a35321750b0f99df18d2
% https://github.com/marverenic/Jockey/commit/647e6d304cced39b7dc18f6195f3258659f72e00
% https://github.com/pf4j/pf4j/commit/f4ddddc61b8643bf4e34ce65b4de9bf2d2bd6831
% 



==> sum.tex <==
We demonstrate {\sc Code2Que}, a web-based tool for improving low-quality question titles in Stack Overflow. 
Developers copy and paste their code snippets into our web application. {\sc Code2Que} automatically generates question titles for the code snippets via a deep sequence-to-sequence model. Developers can utilize the generated questions for their posts. {\sc Code2Que} also searches for related questions with similar problematic code snippets to help developers better understand their problems. Human evaluation results show that for a large number of low-quality questions in Stack Overflow, {\sc Code2Que} can improve the quality of the question titles in terms of \emph{Clearness}, \emph{Fitness}, and \emph{Willingness}. In future work, we will design better models to generate question titles by considering more context information. 
